Theory and Algorithms for Diffusion Processes on Riemannian Manifolds

We study geometric stochastic differential equations (SDEs) and their approximations on Riemannian manifolds. In particular, we introduce a simple new construction of geometric SDEs, using which with bounded curvature. In particular, we provide the first (to our knowledge) non-asymptotic bound on the error of the geometric Euler-Murayama discretization. We then bound the distance between the exact SDE and a discrete geometric random walk, where the noise can be non-Gaussian; this analysis is useful for using geometric SDEs to model naturally occurring discrete non-Gaussian stochastic processes. Our results provide convenient tools for studying MCMC algorithms that adopt non-standard noise distributions.

==> arxiv-appEmbedding.tex <==
\section{Euclidean Embedding}
\label{s:euclidean_embedding}

\subsection{Notation and Assumptions}
\label{ss:euclidean_setup}
In this section, let us $A: \Re^d\to \Sym^{d\times d}$ be a matrix-valued function, and let $g(x):=A^{-1}(x)$. Let us consider the Riemannian manifold $\lrp{\Re^d, g}$, and let $\dist\lrp{x,y}$ be the Riemannian distance for this manifold. 



\begin{assumption}
    \label{ass:g_A_regularity}
    Exist strictly positive constants $\lambda_A, L_A$, such that for all $x,y\in \Re^d$, 
    \begin{alignat*}{1}
        & \lambda_A I \prec A(x) \prec L_A I\\
        & \tr\lrp{A(x) - A(y)}^2 \leq {L_A'}^2 \lrn{x-y}_2^2
    \end{alignat*}
\end{assumption}
\begin{assumption}
    \label{ass:g_A_Lipschitz}
    Exist strictly positive constant $L_A'$, such that for all $x,y\in \Re^d$, 
    \begin{alignat*}{1}
        & \tr\lrp{A(x) - A(y)}^2 \leq {L_A'}^2 \lrn{x-y}_2^2
    \end{alignat*}
\end{assumption}
Note that under Assumption \ref{ass:g_A_Lipschitz}, $\lambda_A \lrn{x-y}_2 \leq \dist\lrp{x,y} \leq L_A \lrn{x-y}_2$. It is useful to note that Assumption \ref{ass:g_A_Lipschitz} and using Lemma 1 from \cite{eldan2020clt}, 
\begin{alignat*}{1}
    \tr\lrp{A^{1/2}(x) - A^{1/2}(y)}^2 \leq \frac{{L_A'}^2}{\lambda_A} \lrn{x-y}_2^2\\
    \elb{e:sqrt_A_regularity}
\end{alignat*}

We use $\lin{\cdot,\cdot}$ to denote the inner product wrt $g$, i.e. given $u,v \in T_x M$, $\lin{u,v} = \sum_{i,j=1}^d u_i v_j g_{i,j}(x)$. We use $\linb{u,v}$ to denote the \emph{Euclidean dot product}, i.e. $\linb{u,v} = \sum_{i=1}^d u_i v_i$. It follows that $\lin{u,v} = \linb{u, g(x) v}$.

We will use $\nabla$ to denote the Levi Civita connection. We use the bold version $\nablab$ to denote the \emph{Euclidean derivative} of a function $h: \Re^d \to \Re$, i.e.
\begin{alignat*}{1}
    \frac{d}{dt} f(x + t v) = \linb{\nablab f(x), v}
\end{alignat*}
We will use $e_i$ to denote the basis vectors, e.g. $e_1 = [0,1,0,0...0]$. We will also use $\partial_i f(x) := \lin{\nablab f(x), e_i}$. Similarly, let $\nabla^2 f$ denote the Hessian tensor wrt the Riemannian metric, and $\nablab^2 f$ denote the Hessian wrt Euclidean metric.

We let $\Gamma$ denote the Christoffel symbols of $g$. Specifically,for $i,j,k\in\lrbb{1...d}$,
\begin{alignat*}{1}
    \Gamma^k_{ij}(x) := \frac{1}{2} \sum_{l=1}^d \lrp{\lrp{\lrp{g(x)}^{-1}}_{kl} \lrp{\del_i g_{jl}(x) + \del_j g_{il}(x) - \del_l g_{ij}(x)}}
    \elb{d:christoffel_symbol}
\end{alignat*}
It will also be convenient to define $\Gamma^k(x)$ as the matrix whose $(i,j)^{th}$ entry is $\Gamma^k_{i,j}$. With slight overloading of notation, we define $\phi(x): \Re^d \to \Re^d$ and $\phi(x,v): \Re^d \times \Re^d \to \Re^d$ as follows:
\begin{alignat*}{1}
    & \phi_k(x):= \tr\lrp{\lrp{g(x)}^{-1} \Gamma^k(x)}\\
    & \phi_k(x,v):= v^T \Gamma^k(x) v
    \elb{d:phi_for_christoffel_symbol}
\end{alignat*}

\begin{assumption}
    \label{ass:phi_Gamma_regularity}
    Exist $L_\phi$, $L_{\phi}'$, such that for all $x,y,v\in \Re^d$,
    \begin{alignat*}{1}
        & \lrn{\phi(x,v)}_2 \leq L_{\phi} \lrn{v}_2^2\\
        & \lrn{\phi(x,v) - \phi(y,v)}_2 \leq L_{\phi}' \lrn{x-y}_2 \lrn{v}_2^2\\
        & \lrn{\phi(x,v) - \phi(x,w)}_2 \leq L_{\phi}\lrn{v-w}_2 \lrp{\lrn{v}+\lrn{w}}
    \end{alignat*}
\end{assumption}
\begin{remark}
    The form of assumption \ref{ass:phi_Gamma_regularity} really arises from its definition in \eqref{d:phi_for_christoffel_symbol}. $L_\phi$ and $L_{\phi}'$ can be bounded, for example, if $\Gamma^i_{jk}$ is coordinate-wise bounded and smooth.
\end{remark}



We note a useful characterization of geodesics in terms of coordinates below (see, e.g. Eqn 4.16 of \cite{lee2018introduction}). A curve $x(t) : \Re \to \Re^d$ is a geodesic if and only if, for all $k\in \lrbb{1...d}$,
\begin{alignat*}{1}
    & x''_k(t) = - \sum_{i,j=1}^d \lrp{x'_i(t) x'_j(t) \Gamma^k_{ij} \lrp{x(t)}} = - \phi(x(t),x'(t))\\
    \Leftrightarrow \qquad 
    & x''(t) = \phi(x(t),x'(t))
    \elb{e:geodesic_equation_coordinate_christoffel}
\end{alignat*}

\begin{assumption}
    \label{ass:euclidean_xi_assumption}
    We assume that the random vector field satisfies, for all $x\in \Re^d$,
    \begin{alignat*}{1}
        \E{\xi(x)} = 0 \qquad \E{\xi(x) \xi(x)^T} = A(x)
    \end{alignat*}
\end{assumption}

\begin{assumption}
    \label{ass:beta_lipschitz_euclidean}
    Assume that for all $x,y$, with probability $1$,
    \begin{alignat*}{1}
        & \lrn{\beta(x) - \beta(y)}_2 \leq L_{\beta,2}' \lrn{x-y}_2\\
        & \lrn{\xi(x) - \xi(y)}_2 \leq L_{\xi,2}' \lrn{x-y}_2\\
        & \lrn{\xi(x)}_2 \leq L_{\xi,2}
    \end{alignat*}
\end{assumption}


\subsection{Euclidean Walk to Manifold Walk}
    \label{ss:euclidean_walk_to_manifold_walk}
\begin{lemma}[One Step Error On Euclidean Space]
    \label{l:euclidean_step_to_manifold_step}
    Assume $\beta$ and $\xi$ satisfy Assumption \ref{ass:beta_lipschitz_euclidean} and Assumption \ref{ass:euclidean_xi_assumption}. Assume \ref{ass:phi_Gamma_regularity}, \ref{ass:g_A_regularity} and \ref{ass:g_A_Lipschitz}. Let $x\in \Re^d$ be an arbitrary point and define
    \begin{alignat*}{1}
        & x' = \Exp_{x} \lrp{\delta \beta(x)+ \sqrt{\delta} \xi(x) + \frac{1}{2} \phi(x) }\\
        & \t{x}' = x + \delta \beta(x) + \sqrt{\delta} \xi(x)
    \end{alignat*}
    Then
    \begin{alignat*}{2}
        & \lrn{x' - \t{x}'}_2^2
        &&\leq O\lrp{\delta^6 \lrn{\beta(x)}_2^6 + \delta^2}\\
        &\lrn{x' - \t{x}' + \frac{1}{2} \phi(x,\sqrt{\delta} \xi(x)) - \frac{\delta}{2}\phi(x)}_2
        &&\leq O\lrp{\delta^3 \lrn{\beta(x)}_2^3 + \delta^{3/2}}
    \end{alignat*}
    where $O\lrp{}$ hides polynomial dependence on $L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_\xi$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{l:euclidean_step_to_manifold_step}]
    Let us define the geodesic $y(t) = \Exp_{x} \lrp{t\lrp{\delta \beta(x) + \delta \phi(x) + \sqrt{\delta} \xi(x)}}$ for $t\in[0,1]$. From \eqref{e:geodesic_equation_coordinate_christoffel}, we verify that $y(t)$ satisfies the following second order ODE:
    \begin{alignat*}{1}
        & y(0) = x\\
        & v(0) = \delta \beta(x) + \sqrt{\delta} \xi(x) + \frac{\delta}{2} \phi(x)\\
        & d y(t) = v(t) dt\\
        & d v(t) = - \phi(y(t),v(t))
    \end{alignat*}
    Thus $y(1) = x'$. We will now bound the distance between $\t{x}'$ and $y(1)$.
    \begin{alignat*}{1}
        & \lrn{y(1) - \t{x}'}_2^2\\
        =& \lrn{\int_0^1 v(t) - \delta \beta(x) - \sqrt{\delta} \xi(x) dt}_2^2\\
        =& \lrn{\int_0^1 v(t) - v(0) + \frac{\delta}{2} \phi\lrp{x} dt}_2^2\\
        =& \lrn{\int_0^1 \int_0^t -\phi\lrp{y(s),v(s)} + \delta \phi\lrp{x} ds dt}_2^2\\
        \leq& \int_0^1 \int_0^t \lrn{-\phi\lrp{y(s),v(s)} + \delta \phi\lrp{x}}_2^2 ds dt
        \elb{e:t:woiemffk:1}\\
        \leq& 8 \int_0^1 \int_0^t \lrn{\phi\lrp{y(s),v(s)} - \phi\lrp{y(0),v(s)} }_2^2 + \lrn{\phi\lrp{y(0),v(s)} - \phi\lrp{y(0),v(0)}}_2^2 \\
        &\quad + \lrn{\phi\lrp{y(0),v(0)} - \delta \phi\lrp{x} }_2^2 ds dt
    \end{alignat*}
    We bound each of the terms above. It will first be convenient to establish a uniform bound on $\lrn{v(t)}$, $\lrn{v(t) - v(0)}$ and $\lrn{y(s) - y(0)}$ for all $t$. Notice by definition of the geodesic that $\lrn{v(t)} = \lrn{v(0)}$ (note: this is $g$-norm) for all $t$, equivalently, $v(t)^T g(y(t)) v(t) = g(0)^T g(y(0)) v(0)$ for all $t$. Let us denote, by $L_v := \sup_{t\in[0,1]} \lrn{v(t)}_2$
    \begin{alignat*}{1}
        & L_v \leq \frac{L_A}{\lambda_A} \lrn{v(0)}_2 \leq \frac{L_A}{\lambda_A} \cdot \lrp{\lrn{\delta\beta(x)}_2 + \sqrt{\delta} L_\xi}\\
        & \lrn{v(t) - v(0)}_2 \leq L_\phi L_v^2 \\
        & \lrn{y(s) - y(0)}_2 \leq L_v
    \end{alignat*}
    By Assumption \ref{ass:phi_Gamma_regularity},
    \begin{alignat*}{1}
        & \lrn{\phi\lrp{y(s),v(s)} - \phi\lrp{y(0),v(s)} }_2
        \leq L_\phi' \lrn{y(s) - y(0)}_2 \lrn{v(s)}_2^2 \leq L_\phi' L_v^3\\
        & \lrn{\phi\lrp{y(0),v(s)} - \phi\lrp{y(0),v(0)}}_2
        \leq L_\phi^2 \lrp{\lrn{v(s)}_2 + \lrn{v(0)}_2} \lrn{v(s) - v(0)}_2 \leq 2 L_\phi L_v^3 \\
        & \lrn{\phi\lrp{y(0),v(0)} - \delta \phi\lrp{x} }_2
        \leq L_{\phi} \lrp{\delta d L_A + \delta^2 \lrn{\beta(x)}^2 + \delta L_\xi^2}
    \end{alignat*}

    
    Plugging and simplifying, 
    \begin{alignat*}{1}
        \lrn{y(1) - \t{x}'}_2^2
        \leq& O\lrp{\delta^6 \lrn{\beta(x)}_2^6 + \delta^4 \lrn{\beta(x)}_2^4 + \delta^2}\\
        =& O\lrp{\delta^6 \lrn{\beta(x)}_2^6 + \delta^2}
    \end{alignat*}
    where $O\lrp{}$ hides polynomial dependence on $L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_\xi$.

    We can also bound
    \begin{alignat*}{1}
        & \lrn{\phi\lrp{y(0),v(0)} - \phi\lrp{x,\sqrt{\delta}\xi(x)} }_2
        \leq L_\phi \lrp{L_v + \sqrt{\delta} \lrn{\xi(x)}_2} \lrp{\lrn{\delta \beta(x)}_2 + \delta L_\phi}
    \end{alignat*}

    Next, following the same steps leading up to \eqref{e:t:woiemffk:1},
    \begin{alignat*}{1}
        &\lrn{y(1) - \t{x}' + \frac{1}{2} \phi(y(0),\sqrt{\delta} \xi(x)) - \frac{\delta}{2}\phi(x)}_2\\
        \leq& \int_0^1 \int_0^t \lrn{-\phi\lrp{y(s),v(s)} + \delta \phi\lrp{x}  + \phi(y(0),\sqrt{\delta} \xi(x)) - \delta \phi(x)}_2 ds dt\\
        \leq& \int_0^1 \int_0^t \lrn{\phi\lrp{y(s),v(s)} - \phi\lrp{y(0),v(s)} }_2 + \lrn{\phi\lrp{y(0),v(s)} - \phi\lrp{y(0),v(0)}}_2 \\
        &\quad + \lrn{\phi\lrp{y(0),v(0)} - \phi\lrp{y(0),\sqrt{\delta} \xi(x) }}_2 ds dt\\
        \leq& O\lrp{\delta^3 \lrn{\beta(x)}_2^3 + \delta^2 \lrn{\beta(x)}_2^2 + \delta^{3/2} + \delta^{3/2} \lrn{\beta(x)}_2 + \delta^{3/2}}\\
        =& O\lrp{\delta^3 \lrn{\beta(x)}_2^3 + \delta^{3/2}}
    \end{alignat*}
    where $O\lrp{}$ hides polynomial dependence on $L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_\xi$.

\end{proof}

\begin{lemma}
    \label{l:euclidean_walk_to_manifold_walk}
    Assume $\beta$ and $\xi$ satisfy Assumption \ref{ass:beta_lipschitz_euclidean} and Assumption \ref{ass:euclidean_xi_assumption}. Assume \ref{ass:phi_Gamma_regularity}, \ref{ass:g_A_regularity} and \ref{ass:g_A_Lipschitz}.
    \begin{alignat*}{1}
        & x_{k+1} = \Exp_{x_k} \lrp{\delta \beta(x_k)+ \sqrt{\delta} \xi_k(x_k) + \frac{\delta}{2} \phi(x_k) }\\
        & z_{k+1} = x_k + \delta \beta(z_k) + \sqrt{\delta} \xi_k(z_k)
    \end{alignat*}
    with $x_0 = z_0$. Assume that $K\delta \leq \min\lrbb{\frac{1}{L_{\beta,2}'}, \frac{1}{L_{\xi,2}'}}$, then
    \begin{alignat*}{1}
        \E{\lrn{x_{K} - z_{K}}_2^2} 
        \leq& O\lrp{K\delta^6 \lrp{\sum_{k=0}^{K-1}\E{\lrn{\beta(x_k)}_2^6}}+ K\delta^2}
    \end{alignat*}
    where $O\lrp{}$ hides polynomial dependence on $L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_{\xi,2}$. and where expectation is wrt the randomness in $\xi_0...\xi_{K-1}$.
\end{lemma}
\begin{proof}
    Consider a fixed $k$. Let us define the geodesic $y(t) = \Exp_{x_k} \lrp{t\lrp{\delta \beta(x_k) + \delta \phi(x_k) + \sqrt{\delta} \xi(x_k)}}$ for $t\in[0,1]$. From \eqref{e:geodesic_equation_coordinate_christoffel}, we verify that $y(t)$ satisfies the following second order ODE:
    \begin{alignat*}{1}
        & y_k(0) = x_k\\
        & v_k(0) = \delta \beta(x_k) + \sqrt{\delta} \xi(x_k) + \frac{\delta}{2} \phi(x_k)\\
        & d y_k(t) = v_k(t) dt\\
        & d v_k(t) = - \phi(y_k(t),v_k(t))
    \end{alignat*}
    Thus $y_k(1) = x_{k+1}$. Next, we define $\bar{x}_{k+1} := x_k + \delta \beta(x_k) + \sqrt{\delta} \xi_k(x_k)$. We can apply Lemma \ref{l:euclidean_step_to_manifold_step} to bound
    \begin{alignat*}{2}
        & \lrn{x_{k+1} - \bar{x}_{k+1}}_2^2
        &&\leq O\lrp{\delta^6 \lrn{\beta(x_k)}_2^6 + \delta^2}\\
        &\lrn{x_{k+1} - \bar{x}_{k+1} + \frac{1}{2} \phi(x_k,\sqrt{\delta} \xi_k(x_k)) - \frac{\delta}{2}\phi(x_k)}_2
        &&\leq O\lrp{\delta^3 \lrn{\beta(x_k)}_2^3 + \delta^{3/2}}
        \elb{e:t:ondasod:1}
    \end{alignat*}
    where $O\lrp{}$ hides polynomial dependence on $L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_{\xi,2}$.

    Consider some fixed $k$. From now on, unless otherwise stated, all expectations are wrt $\xi_k$, conditioned on $\xi_0...\xi_{k-1}$. 
    \begin{alignat*}{1}
        & \E{\lrn{x_{k+1} - z_{k+1}}_2^2}\\
        =& \lrn{x_{k} - z_{k}}_2^2 + \linb{x_{k} - z_{k}, \E{x_{k+1} - x_k - (z_{k+1} - z_k)}} + \E{\lrn{x_{k+1} - x_k - (z_{k+1} - z_k)}_2^2}\\
    \end{alignat*}
    We now bound the $\linb{x_{k} - z_{k}, \E{x_{k+1} - x_k - (z_{k+1} - z_k)}}$ term. Notice that
    \begin{alignat*}{1}
        & \E{x_{k+1} - x_k}\\
        =& \E{\bar{x}_{k+1} - x_k +  x_{k+1} - \bar{x}_{k+1}}\\
        =& \E{\delta \beta(x_k) +  x_{k+1} - \bar{x}_{k+1} + \frac{1}{2} \phi(x_k,\sqrt{\delta} \xi_k(x_k)) - \frac{\delta}{2}\phi(x_k) + \sqrt{\delta} \xi_k(x_k)}\\
        =& \E{\delta \beta(x_k) +  x_{k+1} - \bar{x}_{k+1} + \frac{1}{2} \phi(x_k,\sqrt{\delta} \xi_k(x_k)) - \frac{\delta}{2}\phi(x_k)}
    \end{alignat*}
    where the second equality is because $\E{\phi(x_k,\sqrt{\delta} \xi_k(x_k)) - \delta \phi(x_k)} = 0$, and the third inequality is because $\E{\xi_k(x_k)}=0$. We can also verify that $\E{z_{k+1} - z_k} = \delta \beta(z_k)$. Plugging these into $\linb{x_{k} - z_{k}, \E{x_{k+1} - x_k - (z_{k+1} - z_k)}}$, we get
    \begin{alignat*}{1}
        & \linb{x_{k} - z_{k}, \E{x_{k+1} - x_k - (z_{k+1} - z_k)}}\\
        =& \linb{x_{k} - z_{k}, \delta \beta(x_{k}) - \delta \beta(z_{k})} + \linb{x_{k} - z_{k},  \E{x_{k+1} - \bar{x}_{k+1} + \frac{1}{2} \phi(x_k,\sqrt{\delta} \xi_k(x_k)) - \frac{\delta}{2}\phi(x_k)}}\\
        \leq& \delta {L_{\beta,2}'} \lrn{x_k-z_k}_2^2 + \frac{1}{K} \lrn{x_k-z_k}_2^2 + O\lrp{K\delta^6 \lrn{\beta(x_k)}_2^6 + K\delta^{3}}
    \end{alignat*}
    where we use Assumption \ref{ass:beta_lipschitz_euclidean} and Young's inequality from \eqref{e:t:ondasod:1}.

    Finally, we can bound
    \begin{alignat*}{1}
        & \E{\lrn{x_{k+1} - x_k - (z_{k+1} - z_k)}_2^2}\\
        =& \E{\lrn{x_{k+1} -\bar{x}_{k+1} + \bar{x}_{k+1} - x_k - (z_{k+1} - z_k)}_2^2}\\
        \leq& 2\E{\lrn{x_{k+1} -\bar{x}_{k+1}}_2^2} + 2\E{\lrn{\bar{x}_{k+1} - x_k - (z_{k+1} - z_k)}_2^2}\\
        \leq& O\lrp{\delta^6 \lrn{\beta(x_k)}_2^6 + \delta^2} + 2\delta^2 {L_{\beta,2}'}^2 \lrn{x_k - z_k}_2^2 + 2\delta^2 {L_{\beta,2}'}^2 \lrn{x_k - z_k}_2^2 + 2\delta {L_{\xi,2}'}^2 \lrn{x_k - z_k}_2^2
    \end{alignat*}
    where we use \eqref{e:t:ondasod:1} and Assumption \ref{ass:beta_lipschitz_euclidean}.

    Putting everything together, we get
    \begin{alignat*}{1}
        & \E{\lrn{x_{k+1} - z_{k+1}}_2^2}\\
        \leq& \lrp{1 + 2\delta L_{\beta,2}' + 2\delta {L_{\xi,2}'}^2 + \frac{1}{K}}\lrn{x_{k} - z_{k}}_2^2 + O\lrp{K\delta^6 \lrn{\beta(x_k)}_2^6 + K\delta^{3} + \delta^2}
    \end{alignat*}

    Applying the above recursively for $k=0...K-1$, we get
    \begin{alignat*}{1}
        \E{\lrn{x_{K} - z_{K}}_2^2} 
        \leq& \exp\lrp{1 + 2K\delta L_{\beta,2}' + 2K\delta {L_{\xi,2}'}^2} + O\lrp{K\delta^6 \lrp{\sum_{k=0}^{K-1}\E{\lrn{\beta(x_k)}_2^6}} + K^2\delta^{3} + K\delta^2}\\
        =& O\lrp{K\delta^6 \lrp{\sum_{k=0}^{K-1}\E{\lrn{\beta(x_k)}_2^6}} + K^2\delta^{3} + K\delta^2}
    \end{alignat*}
\end{proof}

\subsection{Manifold SDE to Euclidean SDE}
\begin{lemma}\label{l:manifold_sde_to_euclidean_sde}
    Consider the Riemannian manifold $(\Re^d,g)$. Let $\beta$ be a vector field satisfying Assumption \ref{ass:beta_lipschitz}. Given any initial point $x_0$, orthonormal basis $E$ of $T_{x_0}M$, standard Brownian motion $\BB(t)$ and any $T\in \Re^+$, let $x(t):= \Phi(t;x_0,E,\beta,\BB)$ where $\Phi$ is as defined in \eqref{d:x(t)}, $E$ is an arbitrary orthonormal basis of $x(0)$, $\BB$ is a standard Brownian motion over $\Re^d$. Let us also define the Euclidean SDE
    \begin{alignat*}{1}
        d z(t) = \beta(z(t)) dt - \frac{1}{2} \phi(z(t))dt + g(z(t))^{-1/2} d\WW(t)
    \end{alignat*}
    with $z(0) = x(0)$, and where $\WW(t)$ is another standard Brownian motion and $\phi$ is as defined in \eqref{d:phi_for_christoffel_symbol}.

    Then $x$ and $z$ have the same distribution.
\end{lemma}
\begin{proof}
    We will verify that $x(t)$ and $z(t)$ have the same generator. The conclusion follows from Theorem 1.3.6 of \cite{hsu2002stochastic} which states that diffusion measusure with the given generator and initial distribution is unique.

    We have already observed in Lemma \ref{l:Phi_is_diffusion} that $x(t)$ is the diffusion process generated by $L f = \lin{\nabla f, \beta} + \frac{1}{2} \Delta(f)$, where $\Delta$ denotes the Laplace Beltrami operator. We verify that $z(t)$ has the same generator.

    It is important to recall our definition of $\nablab^2, \nablab, \linb{}, \nabla^2, \nabla, \lin{}$ in Section \ref{ss:euclidean_setup}.

    By Ito's Lemma, for any twice continuously differentiable $f$,
    \begin{alignat*}{1}
        d f(z(t)) 
        =& \linb{\nablab f(z(t)), \beta(z(t))} dt - \frac{1}{2}\linb{\nablab f(z(t)), \phi(z(t))} + \frac{1}{2} \tr\lrp{g(z(t))^{-1} \nablab^2 f(z(t))} dt\\
        &\quad + \linb{\nablab f(z(t)), g(z(t))^{-1} d\WW(t)} 
    \end{alignat*}

    By definition of $\linb{}, \nablab, \lin,\nabla$, $\linb{\nablab f(z(t)), \beta(z(t))} = \lin{\nabla f(z(t)), \beta(z(t))}$. 

    Next, we verify that $- \frac{1}{2}\linb{\nablab f(z(t)), \phi(z(t))} + \frac{1}{2} \tr\lrp{g(z(t))^{-1} \nablab^2 f(z(t))} dt = \frac{1}{2} \Delta f (z(t))$. This is because
    \begin{alignat*}{1}
        \Delta f 
        =& \sum_{j,k=1}^d \lrp{g^{-1}}_{j,k} \lrp{\nablab^2 f}_{k,j} - \sum_{j,k,\ell} \lrp{g^{-1}}_{jk} \Gamma^{\ell}_{jk} \lrp{\nabla f}_{\ell}\\
        =& \tr\lrp{g^{-1} \nablab^2 f} + \linb{\nabla f, \phi}
    \end{alignat*}
    where we use the definition of $\phi$ in \eqref{d:phi_for_christoffel_symbol}.

    We have thus verified that
    \begin{alignat*}{1}
        df(z(t)) - \lin{\nabla f(z(t)), \beta(z(t))} - \frac{1}{2} \Delta f(z(t)) = \linb{\nablab f(z(t)), g(z(t))^{-1} d\WW(t)} 
    \end{alignat*}
    is a martingale.
\end{proof}

\subsection{A CLT for Euclidean SDE}
\begin{lemma}\label{l:euclidean_clt}
    Assume $M= \lrp{\Re^d, g}$ satisfies Assumptions \ref{ass:sectional_curvature_regularity}, \ref{ass:ricci_curvature_regularity} and \ref{ass:higher_curvature_regularity}. Let $A = g^{-1}$ satisfy Assumption \ref{ass:g_A_regularity} and \ref{ass:g_A_Lipschitz}. Let $\beta$ and $\xi$ satisfy Assumptions \ref{ass:beta_lipschitz_euclidean} and \ref{ass:euclidean_xi_assumption} (equivalent to Assumption \ref{ass:moments_of_xi}). Let $\phi$ satisfy Assumption \ref{ass:phi_Gamma_regularity}. Let $\beta^g := \beta + \phi$ satisfying Assumption \ref{ass:beta_lipschitz}. Assume that $\beta^g (x^*) = 0$ at some $x^*\in \Re^d$. Let $\xi$ be a vector field and assume there exists constants $L_\xi,L_\xi',L_\xi'',L_\xi'''$ so that Assumption \eqref{ass:regularity_of_xi} holds with probability 1.

    Let $\delta \in \Re^+$ and $K\in \Z^+$, Let $z_0$ be a point, let $\s:=\max\lrbb{1,\dist\lrp{z_0,x^*}}$. Define
    \begin{alignat*}{1}
        & z_{k+1} = z_k + \delta \beta(z_k) + \sqrt{\delta} \xi_k(z_k)
    \end{alignat*}
    and SDE
    \begin{alignat*}{1}
        d y(t) = \beta(y(t))dt + A(y(t))^{1/2} d\WW(t)
    \end{alignat*}
    where $\WW(t)$ is a Brownian motion and where $y(0) = z_0$.
    There exists constant $\C_1$, which depend polynomially on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'',d,\R,L_{\xi,2}',L_{\beta,2}'$, such that for any positive $T \leq \frac{1}{\C_1}$ and $\delta := {T}^3$ and $K:= T/\delta$, there exists a coupling between $y$ and $\hat{y}$, such that 
    \begin{alignat*}{1}
        \E{\lrn{z_K - y(K\delta)}_2} \leq {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\lrn{z_0 - x^*}_2^3}}
    \end{alignat*}
    where $\t{O}$ hides polynomial dependency on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'',d,\R,L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_{\xi,2}',L_{\beta,2}'$.
\end{lemma}
\begin{remark}
    Note that the requirement that $\delta = (K\delta)^3$ means that for $K\delta \epsilon$ error, we need $K\delta = \epsilon^{2}$ and $\delta = \epsilon^6$.
\end{remark}

\begin{proof}[Proof of Lemma \ref{l:euclidean_clt}]
    Let us define
    \begin{alignat*}{1}
        x_{k+1} = \Exp_{x_k}\lrp{\delta \beta(x_k) + \frac{\delta}{2} \phi(x_k)+ \sqrt{\delta} \xi_k(x_k)}
    \end{alignat*}
    By Lemma \ref{l:euclidean_walk_to_manifold_walk},
    \begin{alignat*}{1}
        \E{\lrn{x_{K} - z_{K}}_2^2} 
        \leq& O\lrp{K\delta^6 \lrp{\sum_{k=0}^{K-1}\E{\lrn{\beta(z_k)}_2^6}}+ K\delta^2}
    \end{alignat*}
    By Lemma \ref{l:euclidean_walk_l2_distance_bound_without_dissipativity} and Assumption \ref{ass:beta_lipschitz_euclidean}, 
    \begin{alignat*}{1}
        \E{\lrn{\beta(z_k)}_2^6} 
        \leq& 8{L_{\beta,2}'}^6\E{\lrn{z_k - z_0}_2^6} +  8\E{\lrn{\beta(z_0)}_2^6}\\
        \leq& 2^{11}{L_{\beta,2}'}^6 \lrp{{K^3\delta^6 \lrn{\beta(z_0)}_2^6} +  K^3 \delta^3 L_{\xi,2}^6} + 8\E{\lrn{\beta(z_0)}_2^6}\\
        \leq& 9\E{\lrn{\beta(z_0)}_2^6} + 2^{11}{L_{\beta,2}'}^6 K^3 \delta^3 L_{\xi,2}^6
    \end{alignat*}
    where we assume that $K\delta \leq 1/(32L_{\beta,2}')$. Plugging into the earlier bound from Lemma \ref{l:euclidean_walk_to_manifold_walk},
    \begin{alignat*}{1}
        \E{\lrn{x_{K} - z_{K}}_2^2} 
        \leq& O\lrp{K\delta^6 \lrn{\beta(z_0)}_2^6 + K\delta^2}\\
        =& O\lrp{ \lrp{K\delta}^{15} \lrn{\beta(z_0)}_2^6 + \lrp{K\delta}^4}\\
        =& O\lrp{ \lrp{K\delta}^{15} \lrn{z_0 - x^*}_2^6 + \lrp{K\delta}^4}
    \end{alignat*}
    using the fact that $\delta = (K\delta)^3$ by definition. The last line is because $\lrn{\beta(z_0)}_2 \leq L_{\beta,2}' \lrn{z_0 - x^*}_2 + \lrn{\beta(x^*)}_2 \leq L_{\beta,2}' \lrn{z_0 - x^*}_2 + L_{\phi}$.

    By Lemma \ref{l:euclidean_step_to_manifold_step}, we verify that $y(t)$ has the same distribution as $\hat{y}(t) = \Phi(K\delta;y_0,E,\beta,\BB)$ where $E$ is some orthonormal basis of $T_{y_0} M$ and $\BB(t)$ is a standard Brownian motion. By Theorem \ref{t:main_nongaussian_theorem},
    \begin{alignat*}{1}
        \E{\dist\lrp{\hat{y}_{K},{x}_{K}}} \leq {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\dist\lrp{z_0,x^*}^3}} = {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\lrn{z_0 - x^*}_2^3}}
    \end{alignat*}

    Combining the bounds on $\E{\dist\lrp{\hat{y}_{K},{x}_{K}}}$ and $\E{\lrn{x_{K} - z_{K}}_2^2}$ (which is entirely dominated in the big-O sense), and using Assumption \ref{ass:g_A_regularity}, and recalling that $\hat{y}_K \overset{d}{=} y(K\delta)$, we conclude that there is a coupling between $z$ and $y$ such that
    \begin{alignat*}{1}
        \E{\lrn{z_K - y(K\delta)}_2} \leq {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\lrn{z_0 - x^*}_2^3}}
    \end{alignat*}
    
\end{proof}

\subsection{SGD Stuff}
Let $\S$ denote a set of samples, let $p_\S$ denote the population distribution over $\S$. $\ell(x,s): \Re^d \to \S$ denote a loss function, where $x$ can be viewed as parameterizing a model. We assume that that $\ell$ is bounded in the following sense
\begin{assumption}
    \label{ass:L_ell}
    Exists $L_\ell$ such that for all $s,s' \in \S$,
    \begin{alignat*}{1}
        \lrn{\nablab \ell(x,s) - \nablab \ell(x,s')}_2 \leq L_{\ell}
    \end{alignat*}
\end{assumption}

Let $\S_n = \lrbb{s_1,s_2,...s_n}$, where $s_i$ are sampled i.i.d from $p_\S$. Let $\t{s}_1 \sim p_\S$ be sampled independently of $s_1...s_n$. Let $\t{\S}_n=\lrp{\t{s}_1,s_2...s_n}$, i.e. $\t{\S}_n$ is $\S_n$ with the first sample replaced.

Let
\begin{alignat*}{1}
    & \ell_n (x) := \frac{1}{n} \sum_{i=1}^n \ell(x,s_i)\\
    & \t{\ell}_n = \frac{1}{n} \lrp{\ell(x,s_1) + \sum_{i=2}^n \ell(x,s_i)}
    \elb{d:ell_n}
\end{alignat*}


Let us define the matrix $A_n(x)$ to be the noise covariance of gradient under the empirical distribution over $\S_n$, i.e.
\begin{alignat*}{1}
    A_n(x)
    :=& \frac{1}{n} \sum_{i=1}^n \lrp{\nablab \ell(x,s_i) - \nablab \ell(x)}\lrp{\nablab \ell_n(x,s_i) - \nablab \ell_n(x)}^T\\
    =& \frac{1}{n} \sum_{i=1}^n \nablab \ell(x,s_i) \nablab \ell(x,s_i)^T - \nablab \ell_n(x) \nablab \ell_n(x)^T
    \elb{d:An}
\end{alignat*}
Let $\t{A}_n$ denote the noise covariance of gradient under  under the empirical distribution over $\t{\S}_n$
\begin{alignat*}{1}
    \t{A}_n(x)
    :=& \frac{1}{n} \sum_{i=2}^n \lrp{\nablab \ell(x,s_i) - \nablab \t{\ell}_n(x)}\lrp{\nablab \ell(x,s_i) - \nablab \t{\ell}_n(x)}^T\\
    &\quad + \frac{1}{n} \lrp{\nablab \ell(x,\t{s}_1) - \nablab \t{\ell}_n(x)}\lrp{\nablab \ell(x,\t{s}_1) - \nablab \t{\ell}_n(x)}^T\\
    =& \frac{1}{n} \lrp{\nablab \ell(x,s_1) \nablab \ell(x,s_1)^T + \sum_{i=2}^n \nablab \ell(x,s_i) \nablab \ell(x,s_i)^T} - \nablab \t{\ell}_n(x) \nablab \t{\ell}_n(x)^T
    \elb{d:tAn}
\end{alignat*}

\begin{lemma}\label{l:sgd:An-tAn}
    Let $\ell_n,\t{\ell}_n,A_n,\t{A}_n$ be as defined in \eqref{d:ell_n}, \eqref{d:An} and \eqref{d:tAn} respectively. Under Assumption \ref{ass:L_ell}, for all $x$,
    \begin{alignat*}{1}
        & \tr\lrp{A_n(x) - \t{A}_n(x)}^2 \leq \frac{128 d L_\ell^4}{n^2}\\
        & \tr\lrp{A_n^{1/2}(x) - \t{A}_n^{1/2}(x)}^2 \leq \frac{128 d L_\ell^4}{\lambda_A n^2}\\
        & \lrn{\t{\ell}_n(x) - {\ell}_n(x)}_2 \leq \frac{2L_\ell}{n}
    \end{alignat*}
\end{lemma}
\begin{proof}
We verify that
\begin{alignat*}{1}
    &A_n(x) - \t{A}_n(x)\\
    =& \frac{1}{n}\underbrace{\lrp{\nablab \ell(x,\t{s}_1) - \nablab \t{\ell}_n(x)}\lrp{\nablab \ell(x,\t{s}_1) - \nablab \t{\ell}_n(x)}^T}_{\circled{1}} - \frac{1}{n}\underbrace{\lrp{\nablab \ell(x,{s}_1) - \nablab {\ell}_n(x)}\lrp{\nablab \ell(x,{s}_1) - \nablab {\ell}_n (x)}^T}_{\circled{2}}\\
    &\quad + \frac{1}{n}\sum_{i=2}^n \underbrace{\lrp{\nablab \ell_n(x) - \nablab \t{\ell}_n(x)}\lrp{\nablab \ell(x,s_i) - \nablab \t{\ell}_n(x)}^T}_{\circled{3}} + \underbrace{\lrp{\nablab \ell(x,s_i) - \nablab {\ell}_n(x)}\lrp{\nablab \t{\ell}_n(x) - \nablab {\ell}_n(x)}^T}_{\circled{4}}
\end{alignat*}
Under Assumption \ref{ass:L_ell}, we can bound $\lrn{\circled{1}}_2+\lrn{\circled{2}}_2\leq 8 L_\ell^2$. Furthermore, we verify that $\lrn{\t{\ell}_n(x) - {\ell}_n(x)}_2 \leq \frac{2L_\ell}{n}$, so that $\lrn{\circled{3}}_2 + \lrn{\circled{4}}_2 \leq \frac{8 L_{\ell}^2}{n}$. Put together, we can bound $\lrn{A_n(x) - \t{A}_n(x)}_2 \leq \frac{16 L_\ell^2}{n}$ and thus
\begin{alignat*}{1}
    & \tr\lrp{A_n(x) - \t{A}_n(x)}^2 \leq \frac{128 d L_\ell^4}{n^2}\\
    & \lrn{\t{\ell}_n(x) - {\ell}_n(x)}_2 \leq \frac{2L_\ell}{n}
\end{alignat*}
The bound on $\tr\lrp{A_n^{1/2}(x) - \t{A}_n^{1/2}(x)}^2$ then follows from Lemma 1 of \cite{eldan2020clt}.
\end{proof}



\begin{lemma}\label{l:euclidean_norm_divergence_under_constant_perturbation}
    Let $u(x)$ be a vector field and $F(x)$ be a matrix valued function. Assume that for all $x$, $\lrn{\t{u}(x) - u(x)}_2 \leq \epsilon_u$ and $\lrn{\t{F}(x) - F(x)}_F \leq \epsilon_F$. Assume further that $\lrn{u(x) - u(y)}_2 \leq L_u'\lrn{x-y}_2$ and $\tr\lrp{F(x) - F(y)}^2 \leq {L_{F}'}^2\lrn{x-y}_2^2$. Let
    \begin{alignat*}{1}
        & d x(t) = u(x(t)) dt + F(x(t)) dB_t\\
        & d y(t) = \t{u}(y(t)) dt + \t{F}(y(t)) dB_t
    \end{alignat*}
    initialized at some arbitrary points $x_0$ and $y_0$ respectively.

    Then
    \begin{alignat*}{1}
        \E{\lrn{x(T)-y(T)}_2^2} \leq e^{T \lrp{2L_u' + 2L_F' + 1}} \lrp{\lrn{x(0)-y(0)}_2^2 + 8  T\lrp{\epsilon_u^2 + \epsilon_F^2}}
    \end{alignat*}
\end{lemma}


\begin{proof}
    Let us denote by $v(x) := u(x) - \t{u}(x)$ and $H(x) := F(x) - \t{F}(x)$. By Ito's Lemma,
    \begin{alignat*}{1}
        &\frac{d}{dt} \E{\lrn{x(t)-y(t)}_2^2}\\
        \leq& \E{2\linb{x(t) - y(t), \lrp{u(x(t)) - u(y(t))} dt + \lrp{F(x(t)) - F(y(t))}, dB_t}}\\
        &\quad + \E{2\linb{x(t)-y(t), v(y(t)) dt + H(y(t)) dB_t}}\\
        &\quad + \E{2 \tr\lrp{F(x(t)) - F(y(t))}^2 + 2\tr\lrp{H(y(t))}^2}\\
        \leq& \lrp{2L_u'+ 2L_F'} \E{\lrn{x(t)-y(t)}_2^2} + 2\epsilon_u \E{\lrn{x(t) - y(t)}_2} + 2 \epsilon_H^2
    \end{alignat*}

    For any $T$, we can apply Young's inequality to get
    \begin{alignat*}{1}
        &\frac{d}{dt} \E{\lrn{x(t)-y(t)}_2^2}
        \leq \lrp{2L_u'+ 2L_F' + 1} \E{\lrn{x(t)-y(t)}_2^2} + \epsilon_u^2 + 2 \epsilon_H^2
    \end{alignat*}

    Integrating over $[0,T]$, we get
    \begin{alignat*}{1}
        \E{\lrn{x(T)-y(T)}_2^2} \leq e^{T \lrp{2L_u' + 2L_F' + 1}} \lrp{\lrn{x(0)-y(0)}_2^2 + 8  T\lrp{\epsilon_u^2 + \epsilon_F^2}}
    \end{alignat*}    
\end{proof}


\subsection{Main SGD Result}
\label{ss:main_sgd_result}



\begin{lemma}\label{l:sgd_stability_lemma}
    Assume the same assumptions as Theorem \ref{t:sgd_stability}.
    
    Let $\delta \in \Re^+$, define the sequences
    \begin{alignat*}{1}
        & x_{k+1} = x_k + \delta \ell_n(x_k) + \sqrt{\delta} \xi_k(x)\\
        & \t{x}_{k+1} = \t{x}_k + \delta \t{\ell}_n(\t{x}_k) + \sqrt{\delta} \t{\xi}_k(\t{x}_k)
    \end{alignat*}
    Let $f,\alpha$ be as defined in Theorem \ref{t:langevin_mcmc}. There exists constant $\C_1$, which depend polynomially on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'', \frac{1}{m},d,\R,L_{\xi,2}',L_{\beta,2}'$, such that for any positive \\
    $T \leq \frac{1}{\C_1}\min\lrbb{1, \frac{1}{\lrn{x_0 - x^*}_2^2 + \lrn{\t{x}_0 - \t{x}^*}_2^2}}$ and $\delta := {T}^3$ and $K:= T/\delta$, there exists a coupling between $x$ and $\t{x}$ such that for $j = \lceil \frac{1}{32 T\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \rceil$,
    \begin{alignat*}{1}
        \E{f\lrp{\dist\lrp{x_{jK}, \t{x}_{jK}}}}
        \leq& \exp\lrp{-\alpha jK\delta}f\lrp{\dist\lrp{x_0,\t{x}_0}}\\
        &\quad + {O}\lrp{j\lrp{K\delta}^{3/2}\lrp{1+\E{\lrn{x_{0} - x^*}_2^3 + \lrn{\t{x}_{0} - \t{x}^*}_2^3}} + \frac{\lrp{jK\delta}}{n}}
    \end{alignat*}
    where $\t{O}$ hides polynomial dependency on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'',d,\R,L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_{\xi,2}',L_{\beta,2}', L_{\ell}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{l:sgd_stability_lemma}]
    Under existing assumption on $T$, we assume without loss of further generality that $K\delta = T \leq \frac{1}{32\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}}$. Thus $\frac{1}{32 T \lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \geq 1$, thus $jK\delta := K\delta \lceil\frac{1}{32K\delta\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \rceil \leq 2$. We verify from definition of $j$ that
    \begin{alignat*}{1}
        \frac{1}{32\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \leq j K\delta \leq \frac{1}{16\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}}
        \elb{e:t:jkdelta}
    \end{alignat*}
    This will be useful at several places later in this proof.

    Let us define, for $t\in[0,jK\delta]$,
    \begin{alignat*}{1}
        & d {y}(t) = \beta({y}(t))dt + A({y}(t))^{1/2} d\WW(t)\\
        & d \t{y}(t) = \t{\beta}(\t{y}(t))dt + \t{A}(\t{y}(t))^{1/2} d\t{\WW}(t)\\
        & d \bar{y}(t) = {\beta}(\bar{y}(t))dt + {A}(\bar{y}(t))^{1/2} d\bar{\WW}(t)
    \end{alignat*}
    where $\WW,\t{\WW},\bar{\WW}$ are Brownian motions and where $y(0) = x_0$, $\t{y}(0) = \bar{y}(0) = \t{x}_0$. We can bound
    \begin{alignat*}{1}
        & \E{f\lrp{\dist\lrp{x_{jK}, \t{x}_{jK}}}}\\
        \leq& \E{f\lrp{\dist\lrp{y({jK}\delta), \bar{y}({jK}\delta)}}} + \E{\dist\lrp{y({jK}\delta), x_{jK}}} + \E{\dist\lrp{\bar{y}({jK}\delta), \t{x}_{jK}}}\\
        \leq& \E{f\lrp{\dist\lrp{y({jK}\delta), \bar{y}({jK}\delta)}}} + \E{\dist\lrp{y({jK}\delta), x_{jK}}} + \E{\dist\lrp{\t{y}({jK}\delta),\t{x}_{jK}}} + \E{\dist\lrp{\bar{y}({jK}\delta), \t{y}({jK}\delta)}}
        \elb{e:t:alkmlakmd}
    \end{alignat*}
    By Lemma \ref{l:manifold_sde_to_euclidean_sde}, $y(t) \overset{d}{=} \Phi(K\delta;y(0),E,\beta^g,{\BB})$ and $\bar{y}(t)\overset{d}{=} \Phi(K\delta;\bar{y}(0),\t{E},{\beta}^g,\bar{\BB})$. Therefore, by Lemma \ref{l:g_contraction_without_gradient_lipschitz}, there exists a coupling between $y$ and $\bar{y}$ such that
    \begin{alignat*}{1}
        \E{f\lrp{\dist\lrp{y(jK\delta),\bar{y}(jK\delta)}}}
        \leq& \exp\lrp{-\alpha jK\delta}f\lrp{\dist\lrp{x_0,\t{x}_0}}
    \end{alignat*}
    
    Now consider a fixed $i \leq j$. Define $\hat{x}_{(i+1)K} := \Phi(K\delta; x_{iK}, E^{iK}, \beta^g, \hat{\BB}^{iK})$ where $E^{iK}$ is an orthonormal basis at $T_{x_{iK}} M$ and $\hat{\BB}^{iK}$ is a Brownian motion. From Lemma \ref{l:manifold_sde_to_euclidean_sde} and Lemma \ref{l:euclidean_clt}, $\E{\lrn{x_{(i+1)K} - \hat{x}_{(i+1)K}}_2} \leq {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\lrn{x_{iK} - x^*}_2^3}}$. By Lemma \ref{l:manifold_sde_to_euclidean_sde} and Lemma \ref{l:euclidean_norm_divergence_under_constant_perturbation} with $\epsilon_u = \epsilon_F = 0$ and $L_u' = L_\beta'$ and $L_F'= L_A'/\sqrt{\lambda_A}$, we can bound \\
    $\E{\lrn{\hat{x}_{(i+1)K} - y((i+1)K\delta)}_2} \leq \exp\lrp{K\delta \lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \E{\lrn{x_{iK} - y(iK\delta)}_2}$. Therefore, by triangle inequality,
    \begin{alignat*}{1}
        & \E{\lrn{x_{(i+1)K} - y((i+1)K\delta)}_2}\\
        \leq& \exp\lrp{K\delta \lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \E{\lrn{x_{iK} - y(iK\delta)}_2} +  {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\lrn{x_{iK} - x^*}_2^3}}
    \end{alignat*}
    Applying the above recursively for $i=0... j-1$, and noting that from \eqref{e:t:jkdelta},$jK\delta \lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}\leq 1/16$, 
    \begin{alignat*}{1}
        \E{\lrn{x_{jK} - y(jK\delta)}_2}
        \leq& 8 \sum_{i=0}^{j-1}  {O}\lrp{\lrp{K\delta}^{3/2}\lrp{1+\E{\lrn{x_{iK} - x^*}_2^3}}}\\
        \leq& {O}\lrp{j\lrp{K\delta}^{3/2}\lrp{1+\E{\lrn{x_{0} - x^*}_2^3}}}
    \end{alignat*}
    where the last inequality is because $\E{\lrn{x_{iK} - x^*}_2^3} \leq O\lrp{\lrn{x_0 - x^*}_2^3}$ by Lemma \ref{l:euclidean_walk_l2_distance_bound_without_dissipativity}, and our assumption that $jK\delta \leq \frac{1}{32L_\beta'}$ from \eqref{e:t:jkdelta}.

    By an identical sequence of steps, we can also show that
    \begin{alignat*}{1}
        & \E{\lrn{\t{x}_{jK} - \t{y}(jK\delta)}_2}
        \leq {O}\lrp{j\lrp{K\delta}^{3/2}\lrp{1+\E{\lrn{\t{x}_{0} - \t{x}^*}_2^3}}}
    \end{alignat*}
    Finally, by Lemma \ref{l:sgd:An-tAn}, we can apply Lemma \ref{l:euclidean_norm_divergence_under_constant_perturbation} with $\epsilon_u = \frac{2L_\ell}{n}$, $\epsilon_F = \frac{16\sqrt{d} L_\ell^2}{\sqrt{\lambda_A} n}$ and $L_u' = L_\beta'$ and $L_F'= L_A'/\sqrt{\lambda_A}$, so that
    \begin{alignat*}{1}
        \E{\lrn{\bar{y}(jK\delta)-\t{y}(jK\delta)}_2^2} 
        \leq& e^{jK\delta \lrp{2L_u' + 2L_F' + 1}} \lrp{\lrn{x(0)-y(0)}_2^2 + 8  jK\delta \lrp{\epsilon_u^2 + \epsilon_F^2}}\\
        =& O\lrp{\frac{jK\delta}{n^2}} = O\lrp{\frac{\lrp{jK\delta}^2}{n^2}}
    \end{alignat*}
    The last line is because by \eqref{e:t:jkdelta}, $\frac{1}{jK\delta} \leq 32\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}$. Note: we picked $j$ to ensure that, while $K\delta$ is small, $jK\delta$ is large -- $O(1)$ in terms of various parameters.

    Plugging everything into \eqref{e:t:alkmlakmd}, (applying Jensen's inequality to $\E{\lrn{\bar{y}(jK\delta)-\t{y}(jK\delta)}_2^2}$)
    \begin{alignat*}{1}
        \E{f\lrp{\dist\lrp{x_{jK}, \t{x}_{jK}}}}
        \leq& \exp\lrp{-\alpha TjK\delta}f\lrp{\dist\lrp{x_0,\t{x}_0}}\\
        &\quad + {O}\lrp{j\lrp{K\delta}^{3/2}\lrp{1+\E{\lrn{x_{0} - x^*}_2^3 + \lrn{\t{x}_{0} - \t{x}^*}_2^3}}} + O\lrp{\frac{\lrp{jK\delta}}{n}}
    \end{alignat*}

    This concludes the proof.
\end{proof}

%\ref{ass:g_A_regularity}
%%\ref{ass:g_A_Lipschitz}
%\ref{ass:phi_Gamma_regularity}
%\ref{ass:euclidean_xi_assumption}
%\ref{ass:beta_lipschitz_euclidean}
%\ref{ass:L_ell}
%\ref{ass:euclidean_dissipativity}



\begin{theorem}
    \label{t:sgd_stability}
    Let $\ell(x,s): \Re^d \times \S \to \Re$ denote a loss function. Let $\ell_n,\t{\ell}_n,A_n,\t{A}_n$ be as defined in \eqref{d:ell_n}, \eqref{d:An}, \eqref{d:tAn}. Assume $\ell$ satisfies \ref{ass:L_ell}. Assume exists $L_{\ell}'$ such that for all $x,y,s$, $\lrn{\nablab \ell(x,s) - \nablab \ell(y,s)}_2 \leq L_{\ell}' \lrn{x-y}_2$. Let $\xi$ be a random vector field satisfying Assumptions \ref{ass:beta_lipschitz_euclidean} and \ref{ass:euclidean_xi_assumption} wrt $A$ and $\t{\xi}$ be a random vector field satisfying Assumptions \ref{ass:beta_lipschitz_euclidean} and \ref{ass:euclidean_xi_assumption} wrt $\t{A}$. Let $M= \lrp{\Re^d, g}$ and $\t{M} = \lrp{\Re^d, \t{g}}$, and assume both $M$ and $\t{M}$ satisfy Assumptions \ref{ass:sectional_curvature_regularity}, \ref{ass:ricci_curvature_regularity} and \ref{ass:higher_curvature_regularity}. Let $\phi$ be as defined in \eqref{d:phi_for_christoffel_symbol} wrt $g$ and analogously $\t{\phi}$ be defined wrt $\t{g}$. Assume $\phi$ and $\t{\phi}$ satisfy Assumption \ref{ass:phi_Gamma_regularity}. Let $\beta := \ell_n$ and $\t{\beta} := \t{\ell}_n$. Assume $\beta, \t{\beta}$ satisfy Assumption \ref{ass:euclidean_dissipativity}. Let $\beta^g := \beta + \frac{1}{2}\phi$ and $\t{\beta}^g := \t{\beta} + \frac{1}{2}\t{\phi}$, and assume ${\beta}^g,\t{\beta}^g$ satisfy Assumptions \ref{ass:distant-dissipativity} and \ref{ass:beta_lipschitz}. Finally, assume there exist points $x^*$ and $\t{x}^*$ such that $\ell_n(x^*) = 0$ and $\t{\ell}_n(\t{x}^*)=0$. Let $x_0$ be some point satisfying $\lrn{x_0 - x^*}_2 \leq \R_2$ and let $\t{x}_0$ be some point satisfying $\lrn{\t{x}_0 - \t{x}^*}_2 \leq \R_2$.
    

    Let $\delta >0$ be a stepsize, let $x_0 = \t{x}_0$, and define the processes
    \begin{alignat*}{1}
        & x_{k+1} = x_k + \delta \ell_n(x_k) + \sqrt{\delta} \xi_k(x)\\
        & \t{x}_{k+1} = \t{x}_k + \delta \t{\ell}_n(\t{x}_k) + \sqrt{\delta} \t{\xi}_k(\t{x}_k)
    \end{alignat*}
    Let $f,\alpha$ be as defined in Theorem \ref{t:langevin_mcmc}. There exists constant $\C_3,\C_4$, which depend polynomially on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'', \frac{1}{m},d,\R,L_{\xi,2}',L_{\beta,2}'$, such that for any positive \\
    $T \leq \frac{1}{\C_2}$ and $\delta := {T}^3$ and $K:= T/\delta$, there exists a coupling between $x$ and $\t{x}$ such that for $j = \lceil \frac{1}{32 T\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \rceil$ and for any $i$,
    \begin{alignat*}{1}
        \E{\lrn{x_{ijK} - \t{x}_{ijK}}_2^2}\leq \min\lrbb{ijK\delta, \frac{1}{\alpha}} \cdot O\lrp{\lrp{K\delta}^{1/2}+ \frac{1}{ n}}
    \end{alignat*}
    where ${O}$ hides polynomial dependency on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_\xi''',L_R,L_R',L_R'',d,\R,L_A, \frac{1}{\lambda_A}, L_\phi, L_{\phi}',d,L_{\xi,2}',L_{\beta,2}', L_{\ell}$.
\end{theorem}
\begin{proof}
    Under Assumption \ref{ass:L_ell} and our assumption on $\lambda_A$, we verify that both $A(x)$ and $\t{A}(x)$ satisfy Assumption \ref{ass:g_A_regularity} with $L_A = 4 L_{\ell}^2$. Our assumption on $L_{\ell'}$ implies Assumption \ref{ass:g_A_Lipschitz} holds with $L_A' \leq 4 L_{\ell}^2 {L_{\ell}'}^2$. Note that $\beta$ and $\t{\beta}$ satisfy Assumption \ref{ass:beta_lipschitz_euclidean} with $L_{\beta,2}' \leq L_{\ell}'$, and Assumption \ref{ass:beta_lipschitz} with $L_{\beta}' \leq L_A L_{\ell}'$.


    Let $\s$ denote a radius and let $V_k$ denote the event that $\sup_{i\leq k} \max\lrbb{\lrn{x_{k} - x_2^*}_2,\lrn{\t{x}_{k} - \t{x}_2^*}_2}\geq \s$. Recall that $x_2^*$ is by definition a point with $\ell_n(x_2^*) = 0$ and similarly $\t{x}_2^*$ is a point with $\t{\ell}_n(\t{x}_2^*) = 0$. From Lemma \ref{l:euclidean_walk_l2_distance_bound},
    \begin{alignat*}{1}
        \Pr{\max_{i\leq k}  \lrn{x_{K} - x^*_2}_2^2 \geq \s^2} 
        \leq& 8K\delta m_2 \exp\lrp{\frac{m_2}{64L_{\xi,2}^2} \lrp{2\R_2^2 + \frac{L_{\beta,2}' \R_2^2}{m_2} - \s^2}}\\
        \leq& 8K\delta m_2 \exp\lrp{\frac{m_2}{64L_{\xi,2}^2} \lrp{\frac{4 L_{\beta,2}' \R_2^2}{m_2} - \s^2}}
    \end{alignat*}
    We get the same bound for $\Pr{\max_{i\leq k}  \lrn{\t{x}_{K} - \t{x}^*_2}_2^2 \geq \s^2}$. Together with the second-moment bound from lemma \ref{l:euclidean_walk_l2_distance_bound} and triangle inequality, we verify that for all $k$, $\E{\ind{V_k^c} \lrp{\lrn{x_k - \t{x}_k}_2}} \leq 16K\delta m_2 \exp\lrp{\frac{m_2}{128L_{\xi,2}^2} \lrp{\frac{4 L_{\beta,2}' \R_2^2}{m_2} - \s^2}} \cdot \sqrt{\frac{L_{\beta,2}'\R_2^2}{m} +\frac{2{L_{\xi,2}}^2}{m}}$. We verify that there is a constant $\C_2=poly(L_{\beta,2}',\R_2,\frac{1}{{m_2}},L_{\xi,2})$, such that for any $T$, $\s= \C_2 \log\lrp{1/T}$ gives $\E{\ind{V_k^c} \lrp{\lrn{x_k - \t{x}_k}_2}} \leq \lrp{T}^{3/2}$. \cheng{double check this last statement to see if it still holds since there is an extra $K\delta m_2$ factor.}

    Consider an arbitrary step $k$, and condition on the event $V_k$. Let $\C_1$ be the constant from Lemma \ref{l:sgd_stability_lemma}. We verify using Lemma 25 of \cite{cheng2020stochastic} that any $T \leq \frac{1}{32 \C_1 \C_2^2 \log\lrp{1 + \C_1 \C_2^2}}$ implies that $T \leq \frac{1}{\C_1 \C_2^2 \log\lrp{T}^2} = \frac{1}{C_1 \s^2}$. Therefore, there exists a $\C_3$ such that, under the event $V_k$, $T = \frac{1}{\C_3}$ satisfies the requirement of Lemma \ref{l:sgd_stability_lemma}, which then implies that
    \begin{alignat*}{1}
        &\E{\ind{V_{k+jK}}f\lrp{\dist\lrp{x_{k+jK}, \t{x}_{k+jK}}}}\\
        \leq& \E{\ind{V_{k}}f\lrp{\dist\lrp{x_{k+jK}, \t{x}_{k+jK}}}}\\
        \leq& \ind{V_k}\exp\lrp{-\alpha jK\delta}f\lrp{\dist\lrp{x_k,\t{x}_k}}\\
        &\quad + {O}\lrp{j\lrp{K\delta}^{3/2}\lrp{1+\E{\ind{V_k}\lrp{\lrn{x_{k} - x^*}_2^3 + \lrn{\t{x}_{k} - \t{x}^*}_2^3}}} + \frac{\lrp{jK\delta}}{n}}\\
        =& \ind{V_k}\exp\lrp{-\alpha jK\delta}f\lrp{\dist\lrp{x_k,\t{x}_k}} + {O}\lrp{j\lrp{K\delta}^{3/2} + \frac{\lrp{jK\delta}}{n}}
        \elb{e:t:alskmdal}
    \end{alignat*}
    where the expectation is conditional on randomness up to step $k$, and where $j:= \lceil \frac{1}{32 T\lrp{1 + 2L_A'/\sqrt{\lambda_A} + L_\beta'}} \rceil$ is as defined in Lemma \ref{l:sgd_stability_lemma}.

    The last line follows from the definition of $V_k$, as well as the fact that $\lrn{x_2^* - x^*}_2 + \lrn{\t{x}_2^* - \t{x}^*}_2 = O(1)$, which we verify presently: Assumption \ref{ass:phi_Gamma_regularity} implies $\lrn{\beta(x^*)}_2 \leq L_{\phi}$. If $\lrn{x^* - x_2^*}_2 \geq \R_2$, then we are done. So suppose otherwise. Assumption \ref{ass:euclidean_dissipativity} implies that $L_\phi \lrn{x^* - x_2^*}_2 \geq \linb{\frac{1}{2}\phi(x^*), x^* - x_2^*} \geq m_2 \lrn{x^* - x_2^*}_2^2$, so that $\lrn{x^* - x_2^*}_2 \leq \frac{L_{\phi}}{m_2}$. By identical argument, $V_k$ also implies $\lrn{\t{x}_2^* - \t{x}^*}_2 \leq \R_2 + \frac{L_{\phi}}{m_2}$.

    Applying \eqref{e:t:alskmdal} recursively over $k$ being a integral multiple of $jK$, we get that for any $i$,
    \begin{alignat*}{1}
        &\E{\ind{V_{ijK}}f\lrp{\dist\lrp{x_{ijK}, \t{x}_{ijK}}}}\\
        \leq& \exp\lrp{-\alpha ijK\delta}\E{\ind{V_{0}}f\lrp{\dist\lrp{x_0,\t{x}_0}}} + {O}\lrp{\sum_{r=0}^{i-1} \exp\lrp{-\alpha rjK\delta} \lrp{j\lrp{K\delta}^{3/2} + \frac{\lrp{jK\delta}}{n}}}\\
        =& O\lrp{\frac{1 - \exp\lrp{-\alpha r j K \delta}}{\alpha} \cdot \lrp{\lrp{K\delta}^{1/2}+ \frac{1}{ n}}}\\
        =& \min\lrbb{ijK\delta, \frac{1}{\alpha}} \cdot O\lrp{\lrp{K\delta}^{1/2}+ \frac{1}{ n}}
    \end{alignat*}
    Finally, recall our earlier bound that $\E{\ind{V_k^c} \lrp{\lrn{x_k - \t{x}_k}_2}} \leq \lrp{K\delta}^{3/2} = \min\lrbb{ijK\delta, \frac{1}{\alpha}} \cdot O\lrp{\lrp{K\delta}^{1/2}+ \frac{1}{ n}}$. 
    
    Summing these two bounds, and using the fact that $r \leq O\lrp{\frac{1}{\alpha}}f(r)$ gives our conclusion.


\end{proof}



\subsection{Stability and generalization}\label{ss:gen-gap}
\begin{lemma}\label{lemma:stability}
    For a given geodesically $L-$lipschitz function $\ell$, any n samples $s_1, s_2, ..., s_n$ (distribution free), and two distributions of parameters $x_0 \sim \pi_0, x_1 \sim \pi_1$, we have 
    \begin{align*}
       \mathbb{E}_{x_0 \sim \pi_0, x_1 \sim \pi_1} \left[\tfrac{1}{n}\sum_{i=1}^n \ell(s_i, x_0) - \ell(s_i, x_1)\right] \le L W_{1} {(x_0, x_1)}.
    \end{align*}
\end{lemma}
\begin{proof}
Let $\pi$ be a coupling between $\pi_0$ and $\pi_1$. In other word $\int \pi(x, y) dy = \pi_0(x), \int \pi(x, y) dx = \pi_1(y) $. Then for any such coupling we have
\begin{align*}
       \mathbb{E}_{x_0 \sim \pi_0, x_1 \sim \pi_1} \left[\tfrac{1}{n}\sum_{i=1}^n \lrp{\ell(s_i, x_0) - \ell(s_i, x_1)}\right] &= \inf_{\pi} \mathbb{E}_{ (x_0 , x_1) \sim \pi} \left[\tfrac{1}{n}\sum_{i=1}^n \lrp{\ell(s_i, x_0) - \ell(s_i, x_1)}\right] \\
       &\le \inf_{\pi}  \mathbb{E}_{ (x_0 , x_1) \sim \pi} \left[\tfrac{1}{n}\sum_{i=1}^n L \dist(x_0, x_1)\right] \\
       &= L W_1(x_0, x_1) 
\end{align*}
\end{proof}
\paragraph{Proof for Lemma~\ref{thm:gen-gap}} 
\begin{proof}
Denote $\cA(S)$ as the algorithm output based on dataset $S$. Denote $S' = \{s_1', ..., s_n'\}$, $S^{i} = \{s_1, ..., s_{i-1}, s_i', s_{i+1}, s_n\}$, where $s_i, s_i'$ are independently sampled from the population distribution. Then
\begin{align*}
    \mathbb{E}_{S, S' \cA} \left[\frac{1}{n}\sum_{i=1}^n \ell(s_i', \cA(S)) - \frac{1}{n}\sum_{i=1}^n \ell(s_i, \cA(S))\right] &= \mathbb{E}_{S, \cA} \left[ \mathbb{E}_{s'} \left[\ell(s', \cA(S))\right] - \frac{1}{n}\sum_{i=1}^n \ell(s_i, \cA(S))\right]\\
    &= \mathbb{E}_{S, s_i', \cA} \left[  \frac{1}{n}\sum_{i=1}^n \ell(s_i', \cA(S)) - \frac{1}{n}\sum_{i=1}^n \ell(s_i, \cA(S)) \right]\\
    &= \mathbb{E}_{S, s_i', \cA} \left[  \frac{1}{n}\sum_{i=1}^n \lrp{\ell(s_i', \cA(S)) -  \ell(s_i, \cA(S))} \right]\\
    &= \mathbb{E}_{S, s_i', \cA} \left[  \frac{1}{n}\sum_{i=1}^n \lrp{\ell(s_i, \cA(S^i)) -  \ell(s_i, \cA(S)) }\right] \\
    &\le \mathbb{E}_{S, s_i', \cA} \left[ L W_1(\cA(S^i), \cA(S))\right]
\end{align*}
The first line uses linearity of expectation. The third line is by the fact that $\cA(S)$ is exchangeable in $x_i$ and hence
\begin{align*}
   \mathbb{E}_{S, s_i', \cA} \left[\ell(s_i, \cA(S^i)) \right] =    \mathbb{E}_{S, s_i', \cA} \left[\ell(s_i', \cA(S)) \right].
\end{align*}
The fourth line follows by Lemma~\ref{lemma:stability}. Then the statement follows by upper-bounding $W_1(\cA(S^i)$ by Theorem~\ref{t:sgd_stability}.
\end{proof}

\iffalse %{ skip for now
\subsection{Experiments}\label{ss:exp}
In this section, we run experiments to investigate the correlation between generalization gap, iteration number and total step sizes. To do so, we train a ResNet18 model \citep{he2016deep} on Cifar10 dataset \citep{krizhevsky2009learning}. We compute the the generalization gap (defined as train error subtracted from validation error) during training, and plot the value against the epoch number at training as well as the square root of cumulative step size, defined as $\textstyle\sum_{i=1}^t \eta_t$ where $\eta_t$ is the learning rate at epoch $t$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{exp.png}
    \caption{Generalization gap against epoch number (first row) and the cumulative sum of step sizes (second row). The left column corresponds to constant learning rate $0.01$. The second column linearly decay learning rate from $0.1$ to $0.001$. The right column decays the learning rate by 10 every 30 epochs starting at lr$=0.1$. }\label{fig:exp}
\end{figure}

We summarize the result in Figure~\ref{fig:exp}. We train the ResNet with three different learning rate schedules: constant learning rate, linear decaying learning rate and piece-wise learning rate. The values of the learning rates are described by the color of the dot. We plot the generalization gap as $y$ axis against the epoch-number on the upper row and the square root of the cumulative sum of the step sizes on the bottom row. 

We observe that the generalization gap increase linearly with respect to cumulative step size at the beginning of training and saturates afterwards. This observation validate our generalization analysis in Lemma~\ref{thm:gen-gap}.
\fi %} 











\subsection{Euclidean Tail Bounds}
\begin{assumption}[$L_2$ one-point dissipativity]
    \label{ass:euclidean_dissipativity}
    There exists a $x^*_2 \in \Re^d$ such that $\beta(x^*_2) = 0$. There exist constants $m_2, \R_2$ and for all $x: \lrn{x-x^*_2}_2 \geq \R_2$, 
    \begin{alignat*}{1}
        \linb{\beta(x), x - x_2^*} \leq - m_2 \lrn{x - x_2^*}_2^2
    \end{alignat*}
\end{assumption}
\begin{lemma}\label{l:euclidean_walk_l2_distance_bound_without_dissipativity}
    Let $\beta$ satisfy Assumption \ref{ass:beta_lipschitz_euclidean}. Let
    \begin{alignat*}{1}
        x_{k+1} =  x_k + \beta(x_k) + \sqrt{\delta} \xi_k(x_k)
    \end{alignat*}
    with arbitrary $x_0$. Assume and $K\delta \leq 1/(32L_{\beta,2}')$. Then for all $k$,
    \begin{alignat*}{1}
        \E{\lrn{x_{k} - x_0}_2^{8}} \leq {2^{10}K^4\delta^8 \lrn{\beta(x_0)}_2^8} + 2^{10} K^4 \delta^4 L_{\xi,2}^8
    \end{alignat*} 
\end{lemma}
\begin{proof}
    \begin{alignat*}{1}
        \lrn{x_{k+1} - x_0}_2^2
        =& \lrn{x_{k} - x_0}_2^2 + 2\linb{x_k - x_0, \beta(x_k) + \sqrt{\delta} \xi_k(x_k)} + \lrn{x_{k+1} - x_0}_2^2
    \end{alignat*}
    Notice that 
    \begin{alignat*}{1}
        \linb{x_k - x_0, \beta(x_k)} 
        \leq& 2\delta L_{\beta,2}'\lrn{x_k - x_0}_2^2 + \frac{\delta}{L_{\beta,2}'} \lrn{\beta(x_0)}_2^2
    \end{alignat*}
    and $\lrn{x_{k+1} - x_0}_2^2 \leq 4\delta^2 {L_{\beta,2}'}^2 \lrn{x_{k+1} - x_0}_2^2 + 4\delta^2 \lrn{\beta(x_0)}_2^2 + 4\delta L_{\xi,2}^2 \leq \delta L_{\beta,2}' \lrn{x_{k+1} - x_0}_2^2 + 4\delta^2 \lrn{\beta(x_0)}_2^2 + 4\delta L_{\xi,2}^2 \leq$ by assumption that $\delta \leq 1/(16 L_{\beta,2}')$. Put together,
    \begin{alignat*}{1}
        \lrn{x_{k+1} - x_0}_2^2 \leq \lrp{1 + 2\delta L_{\beta,2}'}\lrn{x_{k} - x_0}_2^2 + \delta^2 \lrn{\beta(x_0)}_2^2 +  2\delta L_{\xi,2}^2 + 2\linb{x_k - x_0, \sqrt{\delta} \xi_k(x_k)}
    \end{alignat*}
    squaring both sides, applying Young's inequality, then squaring both sides again and applying Young's inequality again,
    \begin{alignat*}{1}
        \lrn{x_{k+1} - x_0}_2^8 
        \leq& \lrp{1 + 16 \delta L_{\beta,2}' + \frac{1}{K}}\lrn{x_{k} - x_0}_2^8 + {2^{8}K^3\delta^8 \lrn{\beta(x_0)}_2^8} + 2^8 K^3 \delta^4 L_{\xi,2}^8 + \circled{*}
    \end{alignat*}
    where $\circled{*}$ has 0-mean conditioned on $x_k$. Therefore,
    \begin{alignat*}{1}
        \E{\lrn{x_{k+1} - x_0}_2^8} \leq \lrp{1+ 16 \delta L_{\beta,2}' + \frac{1}{K}} \E{\lrn{x_{k} - x_0}_2^8} + {2^{8}K^3\delta^8 \lrn{\beta(x_0)}_2^8} + 2^8 K^3 \delta^4 L_{\xi,2}^8
    \end{alignat*}
    Applying the above recursively, we get
    \begin{alignat*}{1}
        \E{\lrn{x_{k} - x_0}_2^8} 
        \leq& {2^{10}K^4\delta^8 \lrn{\beta(x_0)}_2^8} + 2^{10} K^4 \delta^4 L_{\xi,2}^8
    \end{alignat*}
\end{proof}

\begin{lemma}\label{l:euclidean_walk_l2_distance_bound}
    Let 
    \begin{alignat*}{1}
        x_{k+1} =  x_k + \beta(x_k) + \sqrt{\delta} \xi_k(x_k)
    \end{alignat*}
    Assume Assumption \ref{ass:euclidean_dissipativity}, Assumption \ref{ass:beta_lipschitz_euclidean}, and $\delta \leq m_2/(16{L_{\beta,2}'}^2)$. Then for all $K$,
    \begin{alignat*}{1}
        & \E{\lrn{x_{K} - x^*_2}_2^2} \leq \frac{L_{\beta,2}'\R_2^2}{m} +\frac{2{L_{\xi,2}}^2}{m}\\
        & \Pr{\max_{k\leq K}  \lrn{x_{K} - x^*_2}_2^2 \geq t^2} \leq 8k\delta m_2 \exp\lrp{\frac{m_2}{64L_{\xi,2}^2} \lrp{2\lrn{x_{0} - x^*_2}_2^2 + \frac{L_{\beta,2}' \R_2^2}{m_2} - t^2}}
    \end{alignat*} 
\end{lemma}
\begin{proof}
    \begin{alignat*}{1}
        \lrn{x_{k+1} - x^*_2}_2^2
        =& \lrn{x_{k} - x^*_2}_2^2 + 2\linb{x_k - x^*_2, \beta(x_k) + \sqrt{\delta} \xi_k(x_k)} + \lrn{x_{k+1} - x^*_2}_2^2
    \end{alignat*}
    Notice that 
    \begin{alignat*}{1}
        \linb{x_k - x^*_2, \beta(x_k)} 
        \leq& \ind{\lrn{x_k - x^*_2}_2 \geq \R_2} \lrp{-\delta m_2 }\lrn{x_k - x^*_2}_2 + \ind{\lrn{x_k - x^*_2}_2 \leq \R_2} \lrp{\delta L_{\beta,2}' }\lrn{x_k - x^*_2}_2\\
        \leq& -\delta m_2\lrn{x_k - x^*_2}_2 + 2\delta L_{\beta,2}'\R_2^2
    \end{alignat*}
    and $\lrn{x_{k+1} - x^*_2}_2^2 \leq 2\delta^2 {L_{\beta,2}'}^2 \lrn{x_{k+1} - x^*_2}_2^2 + 2\delta L_{\xi,2}^2 \leq \delta m_2/2 \lrn{x_{k+1} - x^*_2}_2^2 + 2\delta L_{\xi,2}^2 \leq$ by assumption that $\delta \leq m_2/(16 {L_{\beta,2}'}^2)$. Put together,
    \begin{alignat*}{1}
        \lrn{x_{k+1} - x^*_2}_2^2 \leq \lrp{1- \delta m_2/2}\lrn{x_{k} - x^*_2}_2^2 + \delta L_{\beta,2}' \R_2^2 +  2\delta L_{\xi,2}^2 + 2\linb{x_k - x^*_2, \sqrt{\delta} \xi_k(x_k)}
    \end{alignat*}
    Applying the above recursively gives us our first result.

    We now apply Lemma \ref{l:doob_maximal_2} with
    \begin{alignat*}{1}
        & q_k = \frac{m_2}{32L_{\xi,2}^2} \lrn{x_{k+1} - x^*_2}_2^2 \qquad \eta_k = \frac{m_2}{32L_{\xi,2}^2} \cdot 2\linb{x_k - x^*_2, \sqrt{\delta} \xi_k(x_k)}\\
        & a = - \delta m_2/2 \qquad b =  \frac{m_2}{32L_{\xi,2}^2}\lrp{\delta L_{\beta,2}' \R_2^2 +  2\delta L_{\xi,2}^2} \qquad c = \frac{\delta m_2}{4} \qquad d=0
    \end{alignat*}
    We verify that $a+c<0$, so that
    \begin{alignat*}{1}
        \Pr{\max_{k\leq K} q_{k} \geq t^2} \leq 8K\delta m_2 \exp\lrp{q_0 + \frac{b+d}{\lrabs{a+c}} - \frac{t^2}{2}}
    \end{alignat*}
    Plugging in the terms,
    \begin{alignat*}{1}
        & \Pr{\max_{k\leq K}  \frac{m_2}{32L_{\xi,2}^2} \lrn{x_{K} - x^*_2}_2^2 \geq t^2} \leq 8 K\delta m_2 \exp\lrp{\frac{m_2}{32L_{\xi,2}^2} \lrn{x_{0} - x^*_2}_2^2 + \frac{ L_{\beta,2}' \R_2^2}{32{L_{\xi,2}'}^2} - t^2/2}\\
        \Leftrightarrow \qquad
        & \Pr{\max_{k\leq K}  \lrn{x_{K} - x^*_2}_2^2 \geq t^2} \leq 8 K\delta m_2 \exp\lrp{\frac{m_2}{64L_{\xi,2}^2} \lrp{2\lrn{x_{0} - x^*_2}_2^2 + \frac{L_{\beta,2}' \R_2^2}{m_2} - t^2}}
    \end{alignat*}
\end{proof}

\subsection{Relation to Fokker Planck}
To reduce notation, in this section, all summation will be from $1$ to $d$, and we drop the explicit dependence on $x$ (e.g. $(g(x))^{-1}$ will be written as $g^{-1}$).

In this section, we simplity $\tr\lrp{g^{-1} \Gamma^m}$. From \eqref{d:christoffel_symbol},
\begin{alignat*}{1}
    \tr\lrp{g^{-1} \Gamma^k}
    =& \frac{1}{2} \sum_{i,j,l} \lrp{g^{-1}}_{ij}\lrp{g^{-1}}_{kl}\lrp{\del_i g_{jl} + \del_j g_{il} + \del_l g_{ij}}
\end{alignat*}
By matrix calculus, for any $A: \Re \to \Sym^{d\times d}$, $\frac{d}{dt} \lrp{A(t)}^{-1} = - A(t)^{-1} \frac{d}{dt} A(t) A(t)^{-1}$, so that the first term of \eqref{d:christoffel_symbol} is simply
\begin{alignat*}{1}
    \sum_{i} \lrp{\sum_{j,l} \lrp{g^{-1}}_{ij} \lrp{g^{-1}}_{kl} \del_i g_{jl}} = \sum_{i} \lrp{\del_i \lrp{g^{-1}}}_{ik}
\end{alignat*}
By symmetry, the second term is also
\begin{alignat*}{1}
    \sum_{j} \lrp{\sum_{i,l} \lrp{g^{-1}}_{ij} \lrp{g^{-1}}_{kl} \del_j g_{il}} = \sum_{j} \lrp{\del_j \lrp{g^{-1}}}_{jk} = \sum_{i} \lrp{\del_i \lrp{g^{-1}}}_{ik}
\end{alignat*}
By matrix calculus, for any $A: \Re \to \Sym^{d\times d}$, $\frac{d}{dt} \log \det\lrp{A(t)}= \tr\lrp{A(t)^{-1} \frac{d}{dt} A(t)}$, so that the third term of \eqref{d:christoffel_symbol} is 
\begin{alignat*}{1}
    \sum_{l} \lrp{g^{-1}}_{kl}\lrp{\sum_{i,j} \del_l g_{ij}\lrp{g^{-1}}_{ij}} = \sum_l \lrp{g^{-1}}_{kl} \del_l \log\det\lrp{g}
\end{alignat*}

==> arxiv-mainbody-retired.tex <==
%\vspace*{-5pt}
\section{Diffusion Approximation of Non-Gaussian walk}
We now study how to approximate the SDE~\eqref{e:intro_sde} by a discrete random walk with non-Gaussian noise. Let $\beta$ be a deterministic and $\xi$ a random vector field $\xi$; given an initial point $y\in M$, we first define
    \begin{alignat*}{1}
        \Psi(\delta;y,\beta,\xi) := \Exp_{y}\bigl(\delta \beta(y) + \sqrt{\delta} \xi(y)\bigr),
        \elb{d:y_k}
    \end{alignat*}
where $\xi$ is a random vector field. Next, we introduce key assumptions on the manifold and the noise.
\begin{assumption}\label{ass:higher_curvature_regularity}
    We assume that the manifold $M$ has Riemannian curvature tensor $R$ satisfying
    \begin{enumerate}
        \item For all $x\in M$, $u,v,w,z,a\in T_x M$, $\lin{(\nabla_a R)(u,v)w,z} \leq L_R'\lrn{u}\lrn{v}\lrn{w}\lrn{z}\lrn{a}$
        \item For all $x\in M$, $u,v,w,z,a,b\in T_x M$, $\lin{(\nabla_b (\nabla_a R))(u,v)w,z} \leq L_R''\lrn{u}\lrn{v}\lrn{w}\lrn{z}\lrn{a}\lrn{b}$
    \end{enumerate}
\end{assumption}
\begin{assumption}[Noise regularity]\label{ass:regularity_of_xi}
    The noise $\xi$ satisfies:
    \begin{inparaenum}[(i)]
        \item $\lrn{\xi(x)} \leq L_{\xi}$;
        \item $\lrn{\lrp{\nabla_{v_1} \xi}(x)} \leq L_{\xi}'$;
        \item $\lrn{\lrp{\nabla_{v_2}\nabla_{v_1} \xi}(x)} \leq L_{\xi}''$;
        \item $\lrn{\lrp{\nabla_{v_3}\nabla_{v_2}\nabla_{v_1} \xi}(x)} \leq L_{\xi}'''$.
    \end{inparaenum}
    for all $x$ and for all $v_1, v_2, v_3 \in T_x M$ satisfying $\lrn{v_1} = \lrn{v_2} = \lrn{v_3} = 1$.
\end{assumption}
\begin{assumption}[Moments of $\xi$]\label{ass:moments_of_xi}
    For all $x\in M$, the noise $\xi$ in satisfies:
    \begin{align*}
        1.\ \E{\xi(x)}=0 \qquad \qquad 2.\ \mathrm{Cov}(\xi(x)) = I.
    \end{align*}
    Specifically, let $E_1,\ldots,E_d$ be any orthonormal basis of $T_x M$. Let $\xib \in \Re^d$ be the coordinates of $\xi$ wrt $E_1,\ldots,E_d$. Then, $\E{\xib(x) \xib(x)^T} = I$.
\end{assumption}
Given these assumptions, we are ready to state the second main result of this paper:
\begin{theorem}\label{t:main_nongaussian_theorem}
    Assume $M$ satisfies Assumptions \ref{ass:sectional_curvature_regularity}, \ref{ass:ricci_curvature_regularity} and \ref{ass:higher_curvature_regularity}. Let $\beta$ be a vector field satisfying Assumption \ref{ass:beta_lipschitz}. Assume in addition that there exists $L_\beta$ such that for all $x\in M$, $\lrn{\beta(x)}\leq L_\beta$. Let $\xi$ be a vector field and assume there exists constants $L_\xi,L_\xi',L_\xi''$ so that Assumption \eqref{ass:regularity_of_xi} holds with probability 1. Assume also that $\xi$ satisfies Assumption \ref{ass:moments_of_xi}. For $k\in \Z^{+}$. 

    There exist a constant $\C_1$, which depend polynomially on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_R,L_R'$, such that for any positive $T \leq \frac{1}{\C_1}$, the following holds:
    
    Let $\delta := {T}^3$ and $K:= T/\delta$. Let $y_0$ be arbitrary, let $x^*$ be any point with $\beta(x^*)=0$. For $k\in \Z^+$, let $y_{k+1} = \Psi(\delta;y_k,\beta,\xi_k)$,where $\Psi$ is as defined \eqref{d:y_k}, and let $\bar{y}_{k} := \bar{\Phi}(k\delta;y_0,E,\beta,\BB,0)$, where $\Phi$ is as defined in \eqref{d:x^i(t)}, $E$ is an orthonormal basis at $T_{y_0}M$, $\BB$ is a standard Euclidean Brownian motion., there is a coupling between $y_K$ and $\bar{y}_K$ for which
    \begin{alignat*}{1}
        \E{\dist\lrp{\bar{y}_{K},y_K}} \leq \t{O}\lrp{T^{3/2} \lrp{1 + L_\beta^2}}
    \end{alignat*}
    where $\t{O}$ hides polynomial dependence on $L_R, L_R', L_\xi, L_\xi', L_\xi'', \log\lrp{\frac{1}{T}}$.
    %$T \leq \min\lrbb{\frac{1}{\C_1},\frac{1}{16\sqrt{L_R} L_\beta' \s}, \frac{\C_u}{L_\beta' \s}, \frac{\C_u^2}{128 L_\xi^2 \log\lrp{1+\s}}, \frac{1}{256 L_R L_\beta' \s^2} ,\frac{d}{L_\beta' \s^2}}$
\end{theorem}

We defer the proof of Theorem \ref{t:main_nongaussian_theorem} to Appendix \ref{s:proof_of_t:main_nongaussian_theorem}.

\vspace*{-5pt}
\subsection{Discussion of Theorem \ref{t:main_nongaussian_theorem}}
Theorem \ref{t:main_nongaussian_theorem} provides a quantitative bound between a discrete semimartingale on $M$ and a diffusion process on $M$. Notably, the noise in the discrete semimartingale is given by a random function $\xi$, whose probability need \emph{not} be rotationally invariant, and hence not invariant wrt parallel transport. We do assume $\xi$ has identity covariance, and bounded Lipschitz derivatives up to third order. 

Corollary \ref{c:theorem_2_corollary} shows how the bound in Theorem \ref{t:main_nongaussian_theorem} leads to a mixing result by combining it with Lemma \ref{l:g_contraction_without_gradient_lipschitz}. In Section \ref{s:SGD}, we use this result to analyze stability of a family of stochastic gradient algorithms.



\begin{corollary}
    \label{c:theorem_2_corollary}
    Assume $M,\beta,\xi$ satisfy the same assumptions as Theorem \ref{t:main_nongaussian_theorem}. Further let $\beta$ satisfy Assumption \ref{ass:distant-dissipativity} with $m,q,\R$, satisfying $m \geq 2L_{\Ric}$, and $q + L_{\Ric} \geq 0$. Let $f,\alpha$ be as in Theorem \ref{t:langevin_mcmc}. 
    
    Let $T\in \Re^+$. Let $\delta := {T}^3$ and $K:= T/\delta$. Let $x^*$ be any point with $\beta(x^*)=0$. For $k\in \Z^+$, let $y_{k+1} = \Psi(\delta;y_k,\beta,\xi_k)$,where $\Psi$ is as defined \eqref{d:y_k}. For $i\in \Z^+$, let $x_{k+1} := \Phi(K\delta;x_{iK},{F^{iK}},\beta,\BB^{iK})$, where $\Psi$ is as defined in  \eqref{d:y_k} and $\Phi$ is defined by~\eqref{d:x(t)}, $F^{iK}$ is an orthonormal basis at $T_{x_{iK}}M$, and $\BB^{iK}$ are independent Brownian motions. Assume that $\dist\lrp{x_0,x^*} \leq 2\R$ and $\dist\lrp{y_0,x^*}\leq 2\R$.
    
    For any $N$, there exist a constant $\C_2$, which depends polynomially on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_R,L_R',d,\R,\log N$, such that if $T \leq \frac{1}{\C_2}$, then there is a coupling between $x_{NK}$ and $y_{NK}$ satisfying
    \begin{alignat*}{1}
        \E{\dist\lrp{x_{NK},{y}_{NK}}}
        \leq \exp\lrp{-\alpha N K\delta + \lrp{q + L_{Ric}}\R^2}\dist\lrp{x_{0},y_{0}} + \exp\lrp{\lrp{q + L_{Ric}}\R^2} \cdot \t{O}\lrp{\delta^{1/6}},
    \end{alignat*}
    where $\t{O}$ hides polynomial dependency on $L_\beta,L_\beta', L_\xi,L_\xi',L_\xi'',L_R,L_R',L_R'', \frac{1}{m},d,\R,\log{N},\log\frac{1}{\delta}$.
\end{corollary}
We defer the proof of Corollary \ref{c:theorem_2_corollary} to Appendix \ref{s:proof_of_t:main_nongaussian_theorem}.

\begin{remark} Observe that for $y_{iK}$ to be $\epsilon$-close to $x_{iK}$ in Wasserstein distance, $\delta$ needs to be order of $\epsilon^6$. The first term requires number of steps $NK = \t{O}\lrp{\log(1/\epsilon)/\delta} = \t{O}\lrp{\epsilon^{-6}}$.
\end{remark}

\subsection{Proof Sketch and Theoretical Contributions}
Below, we sketch the proof of Theorem~\ref{t:main_nongaussian_theorem}, on a high level, there are two steps:
\begin{enumerate}
\setlength{\itemsep}{-1pt}
    \item Define $\bar{y}_{K} := \Exp_{y_0}\lrp{K\delta \beta(y_0) + \sqrt{K \delta} \zeta}$ where $\zeta \sim \N_{y_0}\lrp{0,I}$, i.e. $\bar{y}_K$ is a single Euler Murayama step, of stepsize $K\delta$. We show that, conditioned on $\xi_0,\ldots,\xi_{K-1}$, there is some coupling between $\zeta$ and $\xi_{0},\ldots,\xi_{K -1}$, such that
    $\E{\dist\lrp{y_{K},\bar{y}_{K}}} = \t{O}\lrp{\lrp{K\delta}^{3/2}}$.
    \item We now bound the distance between $\bar{y}_{K}$ and the exact SDE $\hat{y}_{K} := \Phi(K\delta;y_{0},{E},\hat{\BB}^i)$. By Lemma \ref{l:discretization-approximation-lipschitz-derivative}, $\E{\dist\lrp{\bar{y}_{K},\hat{y}_{K}}} \leq \t{O}\lrp{\lrp{K\delta}^{3/2}}$.
\end{enumerate}
Theorem \ref{t:langevin_mcmc} follows by triangle inequality. The main difficulty in the proof is in Step 1. We provide further details below. \emph{To simplify matters, we will sketch the proof of Step 1 while assuming that $\beta=0$ (the main bottleneck in the approximation bound is due to the $\xi$ term).} There are two parts that make up the proof of Step 1.

\textbf{Part 1: A Random Walk over $T_{y_0} M$}\\
Our first step is to construct a discrete stochastic process $\t{z}_k$ in $T_{y_0} M$, such that $\t{y}_k:=\Exp_{z_k}$ approximates $y_k$ for $k=0...K$. This corresponds to Step 1 in the proof of Theorem \ref{t:main_nongaussian_theorem} in Section \ref{s:proof_of_t:main_nongaussian_theorem}. Specifically, $\t{z}_k$ and $\t{y}_k$ are defined as 
\begin{alignat*}{1}
    & \t{y}_0 = y_0, \qquad \t{z}_0 = 0,\\
    & \gamma_k(t) = \Exp_{\t{y}_0} \lrp{(1-t) \t{z}_k}, \quad
     \t{z}_{k+1} = \t{z}_k + \sqrt{\delta} \party{\gamma_k(t)}{}\lrp{\xi_k (\t{y}_k)}, 
    \quad \t{y}_{k+1} = \Exp_{y_0} \lrp{\t{z}_{k+1}}.
    \elb{d:ty_k:main_discussion}
\end{alignat*}
We can apply Corollary \ref{c:K-step-retraction-bound-yk} to bound
\begin{alignat*}{1}
    \E{\dist\lrp{\t{y}_{K},y_{K}}} \leq \t{O}\lrp{\lrp{K\delta}^{3/2}}
    \elb{e:t:sdasd:0}
\end{alignat*}
The key to proving the above inequality is Lemma \ref{l:triangle_distortion_G}: given $x,x' \in M$, and $u = \Exp_{x}^{-1}(x')$ and any $v\in T_x M$, there exists a tensor $G$, that depends only on $x$, such that $\dist\lrp{\Exp_{x}(u+v), \Exp_{x'}(\party{x}{x'}G(v))}\leq O\lrp{\lrn{u}^2\lrn{v}^4}$. Furthermore, $\lrn{G - Id} = O\lrp{\lrn{u}^2}$.

For the purpose of proving Corollary \ref{c:K-step-retraction-bound-yk}, consider each step $k$, and let $x = y_0, x' = \t{y}_k, u = \t{z}_k, v = \party{\t{y}_k}{y_0} \lrp{\sqrt{\delta}\xi_k\lrp{\t{y}_k}}$. With high probability, $\lrn{u}^2 \leq O\lrp{K\delta}$ and $\lrn{v}^2 \leq O\lrp{\delta}$, so that $O\lrp{\lrn{u}^2\lrn{v}^4} = O\lrp{K\delta^3}$. Lemma \ref{l:triangle_distortion_G} thus guarantees that
\begin{alignat*}{1}
    \dist\lrp{\t{y}_{k+1}, \Exp_{\t{y}_{k}}\lrp{\sqrt{\delta} G(\xi(\t{y}_k))}}^2\leq O\lrp{K\delta^3}
    \elb{e:t:sdasd:1}
\end{alignat*}
On the other hand, we can use a basic "synchronous-coupling-like" analysis (Lemma \ref{l:discrete-approximate-synchronous-coupling}) to show that
\begin{alignat*}{1}
    & \E{\dist\lrp{y_{k+1}, \Exp_{\t{y}_{k}}\lrp{\sqrt{\delta} G(\xi(\t{y}_k))}}^2} \\
    \lesssim& \lrp{1+\delta}\E{\dist\lrp{y_{k}, \t{y}_k}^2} - 2\sqrt{\delta} \E{\lin{\Exp_{\t{y}_k}^{-1}, G(\xi_k(\t{y}_k)) - \party{y_k}{\t{y}_k} \xi_k(y_k)}} + \delta \E{\lrn{G(\xi_k(\t{y}_k)) - \party{y_k}{\t{y}_k} \xi_k(y_k)}^2}\\
    \leq& \lrp{1+\delta}\E{\dist\lrp{y_{k}, \t{y}_k}^2} + K^2 \delta^3
    \elb{e:t:sdasd:2}
\end{alignat*}
Note that the above is simplified and keeps only the $K$ and $\delta$ dependence. The last line uses the fact that $1. \E{\xi_k(x)} = 0$, $2. G(v)$ is linear in $v$, and $3. \lrn{G - Id}^2 \leq O\lrp{\lrn{u}^4} = O\lrp{K^2\delta^2}$. Combining \eqref{e:t:sdasd:1} and \eqref{e:t:sdasd:2}, and recursing over $k= K...0$ gives \eqref{e:t:sdasd:0}. Detailed steps can be found in the proof of Corollary \ref{c:K-step-retraction-bound-yk}.

Lemma \ref{l:triangle_distortion_G} is similar to Lemma 3 of \cite{sun2019escaping}, which we restate as Lemma \ref{l:triangle_distortion} in the appendix. Roughly speaking, this result bounds $\dist\lrp{\Exp_{x}(u+v), \Exp_{x'}(\party{x}{x'}G(v))}\leq O\lrp{\lrn{u}^2\lrn{v}^2 \lrp{\lrn{u}^2 + \lrn{v}^2}}$, which ends up being $O\lrp{K^2 \delta^3}$. Compared with \eqref{e:t:sdasd:1}, we see that there is an additional factor of $K$, which would eventually lead to a bound of $O\lrp{K^2 \delta^{3/2}}$ instead of \eqref{e:t:sdasd:0}. The essential difference is our bound is that we pull out the linear error term $G()$ separately; later on, when bounding \eqref{e:t:sdasd:2}, the cross term involving $G(\xi(\cdot))$ has $0$ expectation due to linearity, so that it does not pose an issue. We believe that Lemma \ref{l:triangle_distortion_G} may be of independent interest when one needs to analyze retractions of semimartingales in other settings.

%From Lemma \ref{l:discrete-approximate-synchronous-coupling}, the above is bounded by 
%\begin{alignat*}{1}
%    \lrp{1 + c} \dist\lrp{y_k,\t{y}_k}^2 + c'\delta \lrn{\xi_k ({y}_k) - \party{\t{y}_k}{y_k}G_k(\xi_k (\t{y}_k))}^2 + c''\sqrt{\delta} \underbrace{\lin{\Exp_{y_k}^{-1},\xi_k ({y}_k) - \party{\t{y}_k}{y_k}G_k(\xi_k (\t{y}_k))}}_{\circled{*}}
%\end{alignat*}
%where $c$, $c'$ and $c''$ are constants if $y_k$ and $\t{y}_k$ are sufficiently close to $y_0$, which is true with high probability for sufficiently small $K\delta$.


%, so that $\circled{*}$ has $0$ expectation. The second term can be bounded by $2c \delta {L_\xi'}^2 + 2c\delta L_\xi^2 \lrn{G_k - Id}_2^2$. By Lemma \ref{l:inverse_jacobian}, $\lrn{G_k - Id} \leq L_R \lrn{\t{z}_k}^2 = O\lrp{K\delta}$, so that 
%\begin{alignat*}{1}
%    \E{\dist\lrp{y_{k+1}, \Exp_{\t{y}_k}\lrp{\sqrt{\delta} G_k(\xi_k (\t{y}_k))}}^2} \leq \lrp{1 + c \delta}\E{\dist\lrp{y_{k}, \t{y}_k}^2} + O\lrp{K^2 \delta^3}
%    \elb{e:t:sdasd:2}
%\end{alignat*}


\textbf{Part 2: A Central Limit Theorem}\\
Observe that $\t{z}_K$ is the sum of $\sqrt{\delta} \party{\t{y}_k}{y_0}\xi_k(\t{y}_k)$ for $k=0,\ldots,K-1$. We assumed that $\xi_k(x)$ has $0$-mean and identity covariance for all $x$. Lemma \ref{l:identity_covariance_parallel_transport} implies that the parallel transport of $\xi_k$ must also have $0$-mean and identity covariance. If the $\xi_k$'s are independent, we can just apply standard CLT (e.g. \cite{zhai2018high}) to show that $\t{z}_K$ is close to a $\N(0,K\delta I)$. However, each $\xi_k(\t{y}_k)$ depends on $\xi_0(\t{y_0}),\ldots,\xi_{k-1}(\t{y}_{k-1})$, because it depends on $\t{y}_k$. In Lemma \ref{l:clt:main}, we show that the CLT approximation still holds if 1. $\xi_k$'s have the correct covariance, and 2. $\xi_k$'s have bounded derivatives, up to third order. Specifically, Lemma \ref{l:clt:main} guarantees that
\begin{alignat*}{1}
    W_2\lrp{\t{z}_K, \sqrt{K\delta} \zeta} \leq \t{O}\lrp{\delta^{1/2}} = \t{O}\lrp{\lrp{K\delta}\cdot \delta^{1/6}}
\end{alignat*} 
where $\zeta \sim \N(0,I)$, and we use the definition of $\delta = (K\delta)^3$.











==> arxiv-sgd.tex <==
\section{Stochastic Gradient Descent and Generalization Error}
\label{s:SGD}
In this section, we show how our analysis of the diffusion on Riemannian manifold can lead to a generalization bound for SGD. We begin with setting up the notations and explain why SGD can be viewed as a Riemannian diffusion process.

\subsection{Setup}
To distinguish from $\nabla$ (Levi Civita connection), we use the bold version $\nablab$ to denote the \emph{Euclidean derivative} of a function $h: \Re^d \to \Re$, i.e. $\frac{d}{dt} h(x + t v) = \sum_{i=1}^d \lrp{\nablab h(x)}_i \cdot v_i$.

Let $\ell(x,s): \Re^d \times \S \to \Re$ denote a loss function, with $x$ being model parameters (e.g. neural network weights) and $s$ being a sample (e.g. vector of pixel values). Let $\S_n = \{s_1, s_2, s_{n-1}, s_n\}$ denote a set of $n$ i.i.d samples. Let $\ell_n(x) := \frac{1}{n} \sum_{s\in \S_n} \ell(x,s)$ be the expected gradient wrt uniform distribution over the training set. We are interested in the following sequence:
\begin{alignat*}{1}
    x_{k+1} = x_k - \delta \nablab  \ell_n(x_k) +  \sqrt{\delta}\xi_k(x_k),
    \elb{e:sgd_section:noisy_sgd}
\end{alignat*}
where $\xi_k$ are i.i.d random vector fields satisfying $\E{\xi_k(x)}=0$ and 
$\E{\xi_k(x) \xi_k(x)^T} = $ \\ $ \E{\lrp{\nablab \ell(x,s) - \nablab \ell_n(x)}\lrp{\nablab \ell(x,s) - \nablab \ell_n(x)}^T}$. Let us denote $A_n(x) := \E{\xi_k(x) \xi_k(x)^T}$, where expectation is wrt $s\sim Uniform (\S_n)$. Let us also define the following Euclidean SDE, initialized at $y(0) = x_0$:
\begin{alignat*}{1}
    d y(t) = -\nablab \ell_n(y(t))dt + A_n(y(t))^{1/2} d\WW(t)
    \elb{d:sgd_section:euclidean_sde}
\end{alignat*}
where $\WW(t)$ is a Brownian motion in $\Re^d$. We will see in Section \ref{ss:theorem_4_discussion} that $x_k$ in \eqref{e:sgd_section:noisy_sgd} approximates \eqref{d:sgd_section:euclidean_sde}. Finally, let us define the Riemannian manifold $(\Re^d, g)$, where $g$ is the metric tensor, given by $g(x) = A_n(x)^{-1}$, where $A_n(x)$ is the empirical covariance of gradient at $x$ defined earlier. 

Notice that the noise scaling is $\sqrt{\delta}$, whereas in standard SGD, the $0$-mean noise term has scaling $\delta$. In the study of SGD noise and generalization error, various authors \cite{hoffer2017train,cheng2020stochastic,li2021validity} have proposed the injection of additional noise into SGD iterates, so that the second moment of the noise term is constant even as stepsize goes to $0$. In a related vein, the "linear-scaling-rule", which suggests to multiply stepsize by $c$ whenever batchsize is multiplied by $c$, also works to effectively maintain a constant ratio for $\frac{\lrn{A_n}_2}{\delta}$.  (\cite{krizhevsky2009learning,goyal2017accurate}, see also the discussion in \cite{li2021validity}) Our motivation here is to analyze these "noisy SGD" variants. We do not specify an explicit form for $\xi$, but only impose various regularity assumptions such as \eqref{ass:regularity_of_xi}. This is so our analysis applies for different noise injection schemes, such as adding the difference of indpendently sampled gradients \cite{cheng2020stochastic,li2021validity}, or multiplying the stochastic gradient by a Gaussian noise \cite{hoffer2017train}.

\subsection{The Generalization Gap from Riemannian Diffusion}
We study the generalization performance of SGD via Riemannian diffusion following the stability approach in ~\cite{bousquet2002stability,hardt2016train}. Recall the definitions of $\S_n = \{s_1, s_2, s_{n-1}, s_n\}$, $\ell_n$, $g_n$, $A_n$ from the previous sections. Let $\t{\S}_n := \{s_1', s_2, s_{n-1}, s_n\}$ be an adjacent set of samples, where $s_1'$ is independently sampled, i.e., $\S_n$ and $\t{\S}_n$ differ only in the first sample.
%Let $\S_n$ and $\t{\S}_n$ be two adjacent sets of samples such that ${\S}_n := \{s_1, s_2, s_{n-1}, s_n\}$ and  $\t{S}_n := \{s_1', s_2, s_{n-1}, s_n\}$, where $s_1, ..., s_n, s_1'$ are i.i.d samples. 
Let $\t{\ell}_n$ denote the expected empirical loss on $\S_n$, and let $\t{g}_n(x)$ denote the empirical covariance of $\nablab \ell(x,\cdot)$. Let $\t{A}_n(x) := \t{g}_n(x)^{-1}$. Let $\t{\xi}_k$ be i.i.d random vector fields with $0$-mean and covariance $\t{A}_n(x)$.
\begin{alignat*}{1}
    \t{x}_{k+1} = \t{x}_k - \delta \nablab  \t{\ell}_n(\t{x}_k) +  \sqrt{\delta}\t{\xi}_k(\t{x}_k),
    \elb{e:sgd_section:noisy_sgd_tilde}
\end{alignat*}

\begin{theorem}[Algorithm stability, informal]\label{t:sgd-informal}
    Denote $x_t, x_t'$ as the iterates generated by equation~\ref{e:sgd_section:noisy_sgd} and \ref{e:sgd_section:noisy_sgd_tilde} with data set $\S_n$ and $\S_n'$ respectively. Then for positive integers $K = \mathcal{O}(n^4), \delta = \mathcal{O}(n^{-6})$, we have that for $t = K, 2K, 3K...$, 
    \begin{align*}
        W_1(x_t, x_t') \le \min\{ \mathcal{O}(t\delta n^{-1}), \mathcal{O}(n^{-1})\},
    \end{align*}
    where the hidden constants depend on constants in assumptions but are independent of $n, t, \delta, K$.
\end{theorem}

Detailed theorem statement, along with the assumptions needed, can be found in Theorem~\ref{t:sgd_stability} in Appendix \ref{ss:main_sgd_result}. We discuss Theorem \ref{t:sgd-informal} in more detail at the end in Section \ref{ss:theorem_4_discussion}. Before that, we state the following generalization guarantee on SGD:

\begin{lemma}[Generalization bound]\label{thm:gen-gap}
Denote $x_t,$ as the iterates generated by equation~\ref{e:sgd_section:noisy_sgd} with data set $\S_n$. Then for positive integers $K = \mathcal{O}(n^4), \delta = \mathcal{O}(n^{-6})$, we have that for $t = K, 2K, 3K...$, the generalization gap satisfies
    \begin{align*}
       \mathbb{E}_{S, s' \cA} \bigl[ f(s', x_t) - \frac{1}{n}\sum_{i=1}^n f(s_i, x_t)\bigr] \le \min\{ \mathcal{O}(t\delta n^{-1}), \mathcal{O}(n^{-1})\},
    \end{align*}
    where $s'$ denotes an independent test sample. The hidden constants depend on constants in assumptions but are independent of $n, t, \delta, K$.
\end{lemma}

We highlight that Lemma \ref{thm:gen-gap} captures the dynamics of generalization error during training that the generalization gap first increases from zero and then saturates. In contrast, canonical analysis for generalization error of SGLD~\citep{raginsky2017non} provides a uniform upper bound on generalization gap, whereas the bound in \citep{hardt2016train} is iteration-dependent but keeps increasing during training. Our generalization result achieves the min of both bounds. We provide experimental evidence in Appendix \ref{ss:exp}.



\subsection{Discussion and Proof Outline of Theorem \ref{t:sgd-informal}} \label{ss:theorem_4_discussion}
There are numerous assumptions used in Theorem~\ref{t:sgd-informal}  (see formal statements in Theorem \ref{t:sgd_stability}). They fall into three categories:
\begin{enumerate}[label=\Roman*]
%\setlength{\itemsep}{-1pt}
    \item That $\lambda_A I \prec A(x) \prec L_A I$ (Assumption \ref{ass:g_A_regularity}). This essentially ensures that, up to constants, the Riemannian metric is equivalent to the Euclidean metric. This assumption is satisfied if the covariance matrix of $\xi$ is lower and upper bounded.
    \item That the vector field $\nablab \ell_n(x) + \phi(x)$ ($\phi$ being the trace of the Christoffel symbol defined in \eqref{d:phi_for_christoffel_symbol}) 
    satisfies the \emph{distant-dissipativity} assumption (Assumption \ref{ass:distant-dissipativity}). This is required to apply Lemma \ref{l:g_contraction_without_gradient_lipschitz} in order to show that \eqref{d:sgd_section:euclidean_sde} mixes in Riemannian distance.
    \item Various smoothness assumptions, such as $\lrn{\nablab \ell(x,s) - \nablab \ell(y,s)}_2 \leq L_{\ell}'\lrn{x-y}_2$, $\lrn{\xi(x) - \xi(y)}_2 \leq L_{\xi}' \lrn{x-y}_2$ (Assumption \ref{ass:euclidean_xi_assumption}) and $\tr\lrp{A_n(x) - A_n(y)}^2 \leq {L_A'}^2 \lrn{x-y}_2^2$ (Assumption \ref{ass:g_A_Lipschitz}). These assumptions are satisfied by assuming bounded derivatives of sufficient order on $\ell$ and $\xi$.
\end{enumerate}

The proof of Theorem \ref{t:sgd_stability} can be decomposed as follows: First, in Lemma \ref{l:euclidean_walk_to_manifold_walk}, we show that $x_k$ (as defined in \eqref{e:sgd_section:noisy_sgd}) can be approximated by the sequence $z_{k+1} = \Exp_{z_k} \lrp{- \delta \nablab  \ell_n(x_k) +  \sqrt{\delta}\xi_k(x_k) + \frac{\delta}{2} \phi(z_k)}$, with error $\E{\lrn{x_K - z_K}_2^2} = O\lrp{K\delta^2}$. The $\phi$ is a second-order correction term arising due to interaction between $\sqrt{\delta} \xi$ and the Riemannian curvature. Together with Theorem \ref{t:main_nongaussian_theorem} and Lemma \ref{l:manifold_sde_to_euclidean_sde}, we show in Lemma \ref{l:euclidean_clt} that $\E{\lrn{x_K - y(K\delta)}_2} \leq K\delta \cdot \delta^{1/6}$, where $y(t)$ is as defined in \eqref{d:sgd_section:euclidean_sde}.
    
    
    We highlight that Lemma \ref{l:euclidean_walk_to_manifold_walk} may be of independent interest. For example, the discrete walk in Theorem \ref{t:langevin_mcmc} may not be easily computable on a general manifold. Often, the algorithm has to work in some Euclidean coordinate system, and Lemma \ref{l:euclidean_walk_to_manifold_walk} allows us to approximate one step of \eqref{e:intro:discrete_manifold} by a step in Euclidean coordinates. 

    We repeat Step 1 to show that $\t{x}_{k+1}$ in \eqref{e:sgd_section:noisy_sgd_tilde} is similarly approximated by $d \t{y}(t) = -\nablab \t{\ell}_n(\t{y}(t))dt + \t{A}_n(\t{y}(t))^{1/2} d\WW(t)$. We then define $d \bar{y}(t) = -\nablab \ell_n(\bar{y}(t))dt + {A}_n(\t{y}(t))^{1/2} d\WW(t)$. We show in Lemma \ref{l:euclidean_norm_divergence_under_constant_perturbation} that $\E{\lrn{\t{y}(t) - \bar{y}(t)}_2^2} = O\lrp{t/(n^2)}$. We use Lemma \ref{l:manifold_sde_to_euclidean_sde} to verify that $y$ and $\bar{y}$ are equivalent to SDEs on the manifold $(\Re^d, g)$. Lemma \ref{l:g_contraction_without_gradient_lipschitz} the implies that $\dist\lrp{y(K\delta),\bar{y}(K\delta)}$ contracts in terms of a Lyapunov function (this step crucially relies on II). 
    
    Finally, we remark that as an alternative, we can prove the contraction of $y(K\delta)-\bar{y}(K\delta)$, under assumptions of Euclidean distant-dissipativity instead (see, e.g. Assumption 3.2 of \cite{gorham2019measuring}). Euclidean distant dissipativity is easier to verify, since it is guaranteed by adding a sufficiently strongly convex regularizer outside a ball \cite{cheng2020stochastic}, but may lead to worse mixing rate. We remark that our stability bound in Theorem \ref{t:main_nongaussian_theorem} is unchanged in the big-O sense if we use this approach.



